Predicate Abstraction for Linked Data Structures

We present Alias Refinement Types (ART), a new approach to the verification of correctness properties of linked data structures. While there are many techniques for checking that a heap-manipulating program adheres to its specification, they often require that the programmer annotate the behavior of each procedure, for example, in the form of loop invariants and pre- and post-conditions. Predicate abstraction would be an attractive abstract domain for performing invariant inference, existing techniques are not able to reason about the heap with enough precision to verify functional properties of data structure manipulating programs. In this paper, we propose a technique that lifts predicate abstraction to the heap by factoring the analysis of data structures into two orthogonal components: (1) Alias Types, which reason about the physical shape of heap structures, and (2) Refinement Types, which use simple predicates from an SMT decidable theory to capture the logical or semantic properties of the structures. We prove ART sound by translating types into separation logic assertions, thus translating typing derivations in ART into separation logic proofs. We evaluate ART by implementing a tool that performs type inference for an imperative language, and empirically show, using a suite of data-structure benchmarks, that ART requires only 21% of the annotations needed by other state-of-the-art verification techniques.

==> benchmarkdefs.tex <==
\begin{figure}[t!]
{\small
\begin{align*}
\intertext{{\emph{\bf Types}}}
{\tyapp{list}{\alpha}\tref{p}} \doteq {} &
\qheap{\hplocty{\loc}{t}{\tyapp{list}{\alpha\tref{p\ \code{data}}}\tref{p}}}
 \tybind{h}
        {\tobj{\fld{data}{\alpha},\ \fld{next}{\trefm{\loc}}}}\\
%%
{\tyapp{dll}{\alpha,\beta,\gamma}} \doteq {} &
\qheap{\hplocty{\loc}{t}{\tyapp{dll}{\alpha,\tref{\loc},\beta}}} 
 \tybind{h}
        {\tobj{\fld{data}{\alpha},\ \fld{next}{\trefm{\loc}},\ \fld{prev}{\gamma}}} \\
%%
{\tyapp{clist}{\alpha,\beta}} \doteq {} &
\qheap{\hplocty{\loc}{t}{\tyapp{clist}{\alpha,\beta}}} 
 \tybind{h}
        {\tobj{\fld{data}{\alpha},\ \fld{next}{\tyapp{\fn{Either}}{\tref{\loc},\beta}}}} \\
%%
{\tyapp{tree}{\alpha}\tref{p, q}} \doteq {} &
\exists!\; \hplocty{\loc_{l}}{l}{\tyapp{tree}{\alpha\tref{p\ \code{data}}}\tref{p,q}}
       \hpjoin
       \hplocty{\loc_{r}}{r}{\tyapp{tree}{\alpha\tref{q\ \code{data}}}\tref{p,q}}. \\
& \quad \tybind{t}{\tobj{\fld{data}{\alpha},\ \fld{left}{\trefm{\loc_{l}}},\ \fld{right}{\trefm{\loc_{r}}}}}\\
%%
\tbst{\alpha} \doteq { } & \ttree{\alpha}\tref{(x, \vv) \Rightarrow x \geq \vv, (x, \vv) \Rightarrow x < \vv}\\
%%
\trbt{\alpha} \doteq { } & \exists!\; \hplocty{\loc_{l}}{l}{\fn{eqh}(\alpha, r)}  \hpjoin \hplocty{\loc_{r}}{r}{\fn{eqh}(\alpha, l)}.\\
  &\quad \tybind{t}{\tobj{\fld{color}{\tint},\ \fld{data}{\alpha},\ \fld{left}{\fn{rbp}(\loc_l,l)},\ \fld{right}{\fn{rbp}(\loc_r,r)}}}\\
\fn{eqh}(\alpha,t)    \doteq { } & \reftp{\trbt{\alpha}}{\mheight{\vv} = \mheight{t}} \\
\fn{rbp}(\loc,x)      \doteq { } & \reftp{\trefm{\loc}}{(\code{col} = 1) \Rightarrow \mcolor{x} = 0}
\end{align*}
}%
% \emph{\bf Measures}
% $$\begin{array}{rl>{\ }rl}
%   \fn{keys}(x)      &= \{x.d\} \cup \fn{keys}({x.l}) \cup \fn{keys}({x.r}) &
%   \fn{keys}(\vnull) &= \emptyset \\
%   \mcolor{x}        &= {x.col} &
%   \mcolor{\vnull}   &= 0 \\
%   \mheight{x}       &= (\itex{{x.col} = 0}{0}{1}) + {max}(\mheight{x.l}, \mheight{x.r}) &
%   \mheight{\vnull}  &= 0
%   \end{array}$$
%   \vspace{-\baselineskip}
%   \caption{Data structure and measure definitions}
\label{fig:benchmarkdefs}
\end{figure}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End: 


==> cgencode.tex <==
% \begin{figure}
\def\codesize{\normalsize}
\lstdefinestyle{mycaml}{
   language=Caml,
   % keywordstyle=\codesize\sffamily,
   % identifierstyle=\codesize\sffamily,
   % emphstyle=\codesize\sffamily,
   basicstyle=\codesize\sffamily,
   deletekeywords={with},
   mathescape=true,
   columns=flexible,
   keepspaces=true,
   %% backgroundcolor=\color{lightgray},
   extendedchars=true,
   showstringspaces=false,
   showspaces=false,
   tabsize=2,
   breaklines=true,
   showtabs=false,
   captionpos=b
}

\lstset{style=mycaml}
\begin{figure}
\begin{lstlisting}
CGen : TypeEnv $\times$ HeapEnv $\times$ Stmt $\rightarrow$ {Constr} $\times$ TypeEnv $\times$ HeapEnv

CGen(G,H,s) = match s with
 | x = e $\rightarrow$ let (cs, t) = CGEx(G,H,e) in (cs, x:(Shape(t) $\sqcap$ (v = e));G, H)
 | y = x.f $\rightarrow$ let $\ell$ = loc(G(x)) in ({G $\vdash$ G(x) $<:$ <$\ell$>}, y:TypeAt(H,$\ell$);G,H)
 | x.f = e $\rightarrow$ let (cs, t)     = CGEx(G,H,e)
                  $\ell$          = loc(t)
                  (y:Ty, z) = (H($\ell$), FreshId())
                  ht        = NameFields(z, Ty[f : Shape(t) $\sqcap$ (v = e)])
              in  (cs $\cup$ {G $\vdash$ t $<:$ <$\ell$>}, G, H[$\ell$$\mapsto$z:ht])
 | x = alloc{es} $\rightarrow$ let ($\ell$,z)      = (FreshLoc(), FreshId())
                       (cs,fts) = $\oplus$ {(c,f:t) | (c,t) = CGEx(G,H,e)$\wedge$f:e $\in$ es}
                    in (cs,z:<$\ell$>;G, $\ell$$\mapsto$z:NameFields(z, {fts})*H)
 | pad($\ell$) $\rightarrow$ let (x,T) = (FreshId(), FreshType())
             in  ({G,$\ell$$\mapsto$x:T * H $\vdash$ T}, G, $\ell$$\mapsto$x:T * H)
 | concr(x) $\rightarrow$ let (z, $\ell$)    = (FreshId(), loc(G(x)))
                  (y:Ty)  = H($\ell$)
               in  ({G $\vdash$ G(x) $<:$ <$\ell$>}, y:Ty;G, H[$\ell$$\mapsto$z:Shape(Ty) $\sqcap$ (v = y)])
 | unfold($\ell$) $\rightarrow$ let (x$_c$,T$_c$,H$_c$) = FreshIds(FreshLocs(Expand(G,C[t])))
                in ($\emptyset$, [x/v]InstM(C,x$_c$,H$_c$);G, H[$\ell$$\mapsto$x$_c$:T$_c$]*H$_c$
 | fold($\ell$) $\rightarrow$ let (x:Tx)     = H($\ell$)
                 (Hx,Ho)    = Partition(Reachable(Tx), H $\setminus$ $\ell$)
                 (y,T)      = (FreshId(), FreshType())
                 Tf         = {v:C[T] | InstMeasures(C,x,Hx)}
                 (x:Tc,Hc)  = [T/$\alpha$]InstNames((x:Tx,Hx), Expand(G,C[$\alpha$]))
                 cs         = {G,H $\vdash$ T} $\cup$ FoldHeaps(G,(x,Tx,Hx),(x,Tc,Hc))
             in  (cs, G, $\ell$$\mapsto$x:Tf*Ho)
 | s1;s2 $\rightarrow$ let (cs$_1$, G', H') = CGen(G,H,s1)
                (cs$_2$, G'', H'') = CGen(G',H',s2)
            in  (cs$_1$ $\cup$ cs$_2$, G'', H'')
 | $\mathsf{if}$ e $\mathsf{then}$ s$_1$ $\mathsf{else}$ s$_2$ $\rightarrow$
     let (csg, _)      = CGEx(G,H,e)
         ((cs$_1$, G$_1$, H$_1$), (cs$_2$, G$_2$, H$_2$)) = (CGen(C,e;G,H), CGen(C,$\lnot$e;G,H))
         G'            = Fresh(Shape({x:T | x $\in$ G$_1$ $\wedge$ x $\in$ G$_2$ }))
         H'            = Fresh(Shape(FreshBinders(H$_1$)))
         cs            = ({G';G, H' $\vdash$ G'} $\cup$ {G';G, $\vdash$ H'} 
                       $\cup$ {G$_1$ $\vdash$ H$_1$ $<:$ H'} $\cup$ {G$_2$ $\vdash$ H$_2$ $<:$ H'}
                       $\cup$ {G$_1$ $\vdash$ t$_i$ $<:$ t$_i$' | x$_i$:T$_i$ $\in$ G'} 
                       $\cup$ {G$_2$ $\vdash$ t$_i$ $<:$ t$_i$' | x$_i$:T$_i$ $\in$ G'}
     in  (cs, G', H')
 | $\mathsf{return}$ e $\rightarrow$ let (cs, t)    = CGEx(G,H,e)
                   (H',H'')   = Frame(H,Hr)
                   (xr:tr,Hr) = CurrentReturn(G)
               in  (({G $\vdash$ t $<:$ [e/xr]tr} $\cup$ {G $\vdash$ H $<:$ [e/xr]Hr}, $\mathsf{false}$, $\mathsf{emp}$)
 | x = f(es)) $\rightarrow$
   let (xs, fts, x:T, Hin, Hout) = BreakFunSchema(Inst(GlobalType(f)))
       (Hm, Hu)                  = Frame(H,Hin)
       cs = ⋃ {{c, G $\vdash$ t $<:$ [es/xs]t'} | (c,t) = CGEx(G,H,e), 
                                         (e,x) ∈ (combine(es,xs))}
            $\cup$ { G $\vdash$ Hm $<:$ [es/xs]Hin } 
   in (cs, x:[es/xs]T;G, Hu*[es/xs]Hout)
\end{lstlisting}
\end{figure}

\begin{figure}
\begin{lstlisting}              
FoldHeaps(G,(x,t1,H1),(x,t2,H2)) =
  if locs(T1) $\cap$ dom(H1) = $\emptyset$ then
    { G $\vdash$ t1 $<:$ t2 }
  else match (t1, t2) with
    | ({ v:<$\ell$> | p }, _)) $\rightarrow$
        let ((y,Ty1), (y,Ty2) = (H1($\ell$), H2($\ell$)) in
        {G $\vdash$ t1 $<:$ t2} $\cup$ FoldHeaps(G,(y,Ty1,H1 $\setminus$ $\ell$), (y,Ty2,H2 $\setminus$ $\ell$))
    | ({ v:?<$\ell$> | p }, _) $\rightarrow$
        let ((y,Ty1), (y,Ty2) = (H1($\ell$), H2($\ell$)) in
        { G $\vdash$ t1 $<:$ t2 }
        $\cup$ FoldHeaps(add(x,t1 $\sqcap$ (v $\neq$ null),G),(y,Ty1,H1 $\setminus$ $\ell$), (y,Ty2,H2 $\setminus$ $\ell$))
        $\cup$ FoldHeaps(add(x,t1 $\sqcap$ (v = null),G),(y,Ty1,H1 $\setminus$ $\ell$), (y,Ty2,H2 $\setminus$ $\ell$))
    | ({ v:{ fs1 } | p1 }, { v: { fs2 } | p2}) $\rightarrow$
        let x = FreshId() in 
        $\bigcup$ { FoldHeaps(G,(x,Tf1,H1),(x,Tf2,H2)) |  (f1:Tf1, f2:Tf2) in combine(fs1, fs2)
\end{lstlisting}
\end{figure}
% \caption{Constraint Generation Algorithm}
% \label{fig:cgen}
% \end{figure}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> cgencode_split.tex <==
% \begin{figure}
\lstdefinestyle{mycaml}{
   language=[Objective]Caml,
   keywordstyle={\bfseries\codesize\sffamily},
   % identifierstyle=\codesize\sffamily,
   % emphstyle=\codesize\sffamily,
   basicstyle=\codesize\sffamily,
   deletekeywords={null},
   mathescape=true,
   columns=flexible,
   keepspaces=true,
   %% backgroundcolor=\color{lightgray},
   extendedchars=true,
   showstringspaces=false,
   showspaces=false,
   tabsize=2,
   breaklines=true,
   showtabs=false,
   captionpos=b,
   belowskip=0pt
}
\def\inline{\lstinline[style=mycaml,basicstyle=\normalsize\sffamily]}
\lstset{language=Caml}
\lstset{style=mycaml}

 % | y = x.f $\rightarrow$ let $\ell$ = loc($\ctx$(x)) in ({$\ctx$ $\vdash$ $\ctx$(x) $<:$ <$\ell$>}, y:TypeAt($\heap$,$\ell$);$\ctx$,$\heap$)
\begin{figure}[tb]
\begin{lstlisting}
CGen : FunEnv $\times$ TypeEnv $\times$ HeapEnv $\times$ Stmt $\rightarrow$ {Constr} $\times$ TypeEnv $\times$ HeapEnv
CGen($\Phi$,$\ctx$,$\heap$,s) = match s with
 | x = e $\rightarrow$ let (cs, t) = CGEx($\ctx$,$\heap$,e) in (cs, x:(Shape(t) $\sqcap$ (v = e));$\ctx$, $\heap$)
 | y = x.f $\rightarrow$ let $\ell$ = loc($\ctx$(x)) in ({$\issubtype{\ctx}{}{\ctx(\mathsf{x})}\tref{\loc}$}, y:TypeAt($\heap$,$\ell$);$\ctx$,$\heap$)
 | x.f = e $\rightarrow$ let (cs, t)     = CGEx($\ctx$,$\heap$,e)
                  $\loc$          = Loc(t)
                  (y:T$_{\fn{y}}$, z) = ($\heap$($\loc$), FreshId())
                  ht        = NameFields(z, T$_{\fn{y}}$[f : Shape(t) $\sqcap$ (v = e)])
              in  (cs $\cup$ {$\issubtype{\ctx}{}{\mathsf{t}}{\tref{\loc}}$}, $\ctx$, $\heap$[$\loc \mapsto$z:ht])
 | x = alloc{es} $\rightarrow$ let ($\ell$,z)      = (FreshLoc(), FreshId())
                       (cs,fts) = $\oplus$ {(c,f:t) | (c,t) = CGEx($\ctx$,$\heap$,e)$\wedge$f:e $\in$ es}
                    in (cs,z:<$\ell$>;$\ctx$, $\ell$$\mapsto$z:NameFields(z, {fts})*$\heap$)
\end{lstlisting}
\caption{Statement constraint generation}
\label{fig:cgen1}
\end{figure}

% \begin{figure}[tb]
% \begin{lstlisting}
%   $\ldots$
%  | s1;s2 $\rightarrow$ let (cs$_1$, $\ctx'$, $\heap'$) = CGen($\Phi$,$\ctx$,$\heap$,s1)
%                (cs$_2$, $\ctx''$, $\heap''$) = CGen($\Phi$,$\ctx'$,$\heap'$,s2)
%             in  (cs$_1$ $\cup$ cs$_2$, $\ctx''$, $\heap''$)
%  | $\mathsf{if}$ e $\mathsf{then}$ s$_1$ $\mathsf{else}$ s$_2$ $\rightarrow$
%      let (csg, _) = CGEx($\ctx$,$\heap$,e)
%          ((cs$_1$, $\ctx$$_1$, $\heap$$_1$), (cs$_2$, $\ctx$$_2$, $\heap$$_2$)) = (CGen($\Phi$,e;$\ctx$,$\heap$), CGen($\Phi$,$\lnot$e;$\ctx$,$\heap$))
%          $\ctx'$ = Fresh(Shape({x:T$_1$ | x:T$_1$ $\in$ $\ctx$$_1$ $\wedge$ x:T$_2$ $\in$ $\ctx$$_2$ }))
%          $\heap'$ = Fresh(Shape(FreshBinders($\heap$$_1$)))
%          cs = {$\ctx'$, $\heap'$ $\vdash$ $\ctx'$} $\cup$ {$\ctx'$ $\vdash$ $\heap'$} 
%               $\cup$ {$\issubtype{\ctx_1}{}{\heap_1}{\heap'}$} $\cup$ {$\issubtype{\ctx_2}{}{\heap_2}{\heap'}$}
%               $\cup$ {$\issubtype{\ctx_1}{}{\fn{T}}{\fn{T}'}$ | x:T $\in$ $\ctx_1$ $\wedge$ x:T' $\in$ $\ctx'$} 
%               $\cup$ {$\issubtype{\ctx_2}{}{\fn{T}}{\fn{T}'}$ | x:T $\in$ $\ctx_2$ $\wedge$ x:T' $\in$ $\ctx'$} 
%      in  (cs, $\ctx'$, $\heap'$)
%  | $\mathsf{return}$ e $\rightarrow$ let (cs, t) = CGEx($\ctx$,$\heap$,e)
%                  ($\heap'$,$\heap''$) = Frame($\heap$,$\heap_{\mathsf{r}}$)
%                  (xr:tr,$\heap_{\mathsf{r}}$) = CurrentReturn($\ctx$)
%                in (({$\issubtype{\ctx}{}{\mathsf{t}}{\sub{\mathsf{xr}}{\mathsf{e}}\mathsf{tr}}$} $\cup$ {$\issubtype{\ctx}{}{\heap'}{\heap_{\mathsf{r}}}$}, $\mathsf{false}$, $\mathsf{emp}$)
%  | x = f(es)) $\rightarrow$
%    let (xs, fts, x:T, $\heap_{\fn{in}}$, $\heap_{\fn{out}}$) = BreakFunSchema(Inst($\Phi$(f)))
%        ($\heap_{\fn{m}}$, $\heap_{\fn{u}}$) = Frame($\heap$,$\heap_{\fn{in}}$)
%        ($\theta$, exs) = (MakeSubst(xs $\mapsto$ es), Combine(es,xs))
%        cs = $\bigcup$ {c $\cup$ {$\issubtype{\ctx}{}{\fn{T}}{\theta\fn{T}'}$} | (c,T) = CGEx($\ctx$,$\heap$,e) $\wedge$ (e,x) $\in$ exs}
%             $\cup$ { $\issubtype{\ctx}{}{\heap_{\fn{m}}}{\theta\heap_{\fn{in}}}$ } 
%    in (cs, x:$\theta$T;$\ctx$, $\heap_{\fn{u}}$*$\theta$$\heap_{\fn{out}}$)
% \end{lstlisting}
% \caption{Compound statement and function call constraint generation}
% \label{fig:cgen2}
% \end{figure}

\begin{figure}[tb]
\begin{lstlisting}
  $\ldots$
 | pad($\loc$) $\rightarrow$ let (x,T) = (FreshId(), FreshType())
             in ({$\iswellformed{\ctx,\loc\mapsto\fn{x:T}\hpjoin\heap}{\fn{T}}$, $\ctx$, $\loc\mapsto$x:T$\hpjoin\heap$)
 | concr(x) $\rightarrow$ let (z, $\loc$) = (FreshId(), Loc($\ctx$(x)))
                  (y:T$_{\fn{y}}$) = $\heap$($\loc$)
               in ({$\ctx$ $\vdash$ $\ctx$(x) $<:$ <$\loc$>}, y:T$_{\fn{y}}$;$\ctx$, $\heap$[$\loc$$\mapsto$z:Shape(T$_{\fn{y}}$) $\sqcap$ (v = y)])
 | unfold($\ell$) $\rightarrow$ let (x$_c$,T$_c$,$\heap$$_c$) = FreshIds(FreshLocs(Expand($\ctx$,C[t])))
                in ($\emptyset$, $\sub{\vv}{\fn{x}}$InstM(C,x$_c$,$\heap$$_c$);$\ctx$, $\heap$[$\ell$$\mapsto$x$_c$:T$_c$]*$\heap$$_c$
 | fold($\loc$) $\rightarrow$ let (x:T$_{\fn{x}}$) = $\heap$($\loc$)
                 ($\heap_{\fn{x}}$,$\heap_{\fn{o}}$) = Partition(Reachable(T$_{\fn{x}}$), $\heap$ $\setminus$ $\loc$)
                 (y,T) = (FreshId(), FreshType())
                 (x:T$_{\fn{c}}$,$\heap_{\fn{c}}$) = [T/$\alpha$]InstNames((x:T$_{\fn{x}}$,$\heap_{\fn{x}}$), Expand($\ctx$,C[$\alpha$]))
                 T$_{\fn{f}}$ = {$\vv$:C[T] | InstMeasures(C,x,$\heap_{\fn{x}}$)}
                 cs = {$\ctx$,$\heap$ $\vdash$ T} $\cup$ FoldHeaps($\ctx$,(x,T$_{\fn{x}}$,$\heap_{\fn{x}}$),(x,T$_c$,$\heap_{\fn{c}}$))
             in  (cs, $\ctx$, $\loc$$\mapsto$x:T$_{\fn{f}}$*$\heap_{\fn{o}}$)
\end{lstlisting}
\caption{Annotation constraint generation}
\label{fig:cgen3}
\end{figure}

\begin{figure}[tb]
\begin{lstlisting}              
FoldHeaps($\ctx$,(x,$\vsub{T}{1}$,$\heapss{1}$),(x,$\vsub{T}{2}$,$\heapss{2}$)) =
  { $\issubtype{\ctx}{}{\vsub{T}{1}}{\vsub{T}{2}}$ } $\cup$
  if locs($\vsub{T}{1}$) $\cap$ dom($\heapss{1}$) = $\emptyset$ then $\emptyset$ else
  match ($\vsub{T}{1}$, $\vsub{T}{2}$) with
    | ({ v:<$\ell$> | p }, _)) $\rightarrow$ let ((y:$\vsub{T}{y1}$), (y:$\vsub{T}{y2}$) = ($\heapss{1}$($\ell$), $\heapss{2}$($\ell$))
                            in FoldHeaps($\ctx$,(y,$\vsub{T}{y1}$,$\heapss{1}$ $\setminus$ $\ell$), (y,$\vsub{T}{y2}$,$\heapss{2}$ $\setminus$ $\ell$))
    | ({ v:?<$\ell$> | p }, _) $\rightarrow$
        let ((y,$\vsub{T}{y1}$), (y,$\vsub{T}{y2}$) = ($\heapss{1}$($\ell$), $\heapss{2}$($\ell$))
        in  FoldHeaps(add(x,$\vsub{T}{1}$ $\sqcap$ (v $\neq$ null),$\ctx$),(y,$\vsub{T}{y1}$,$\heapss{1}$ $\setminus$ $\ell$), (y,$\vsub{T}{y2}$,$\heapss{2}$ $\setminus$ $\ell$))
         $\cup$ FoldHeaps(add(x,$\vsub{T}{1}$ $\sqcap$ (v = null),$\ctx$),(y,$\vsub{T}{y1}$,$\heapss{1}$ $\setminus$ $\ell$), (y,$\vsub{T}{y2}$,$\heapss{2}$ $\setminus$ $\ell$))
    | ({ v:{ fs1 } | p1 }, { v: { fs2 } | p2}) $\rightarrow$
        let (x, fs) = (FreshId(), combine(fs1, fs2)) in 
        $\bigcup$ { FoldHeaps($\ctx$,(x,Tf1,$\heapss{1}$),(x,Tf2,$\heapss{2}$)) |  (f1:Tf1, f2:Tf2) $\in$ fs }
\end{lstlisting}
\caption{Heap folding constraint generation}
\label{fig:cgen4}
\end{figure}
% \caption{Constraint Generation Algorithm}
% \label{fig:cgen}
% \end{figure}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> check-interp.tex <==
\begin{figure}
\begin{align*}
  \denote{\exprtype{\ctx}{\heap}{\expr}{\ty}{\heap'}}
  & = \validimp{\denote{\ctx}\wedge\denote{\heap}}{\sprop{\tau}{\expr}}
  \\
  %
  \denote{\issubtype{\ctx}{\heap}
                    {\reftp{\tbase}{\pred}}
                    {\reftp{\tbase}{\pred'}}}
  & = \validimp{\denote{\ctx}\wedge\denote{\heap}\wedge\denote{\pred}}
               {\denote{\pred'}}
  \\
  %
  \denote{\stmttype{\ctx}{\heap}{\stmt}{\ctx'}{\heap'}}
  & = \htriplec{\denote{\Phi}\wedge\denote{\ctx}\wedge\denote{\heap}}
               {\stmt}
               {\denote{\ctx'}\wedge\denote{\heap'}}
\end{align*}
\caption{Interpretation of type judgements}
\label{fig:interp-judge}
\end{figure}

\begin{figure*}
  \[
\inference{
  \denote{\ctx}\wedge\denote{\heap} = R\hpjoin \sepmap{\loc}{y}
&
  \inference{
   \htriplec{\sepmap{\loc}{y}}{\conc{\loc}}{\sepmap{\loc}{y}}
  }{
   \htriplec{R\hpjoin\sepmap{\loc}{y}}{\conc{\loc}}{R\hpjoin\sepmap{\loc}{y}}
  }
  &
  \denote{\ctx}\wedge\denote{\heap} 
    \Rightarrow 
\denote{{\tybind{y}{\ty_y}};\ctx} \wedge \denote{\hplocty{\loc}{\tybind{y'}{\ty_{y'}}} \hpjoin \heap'}
  \\
}{
  \htriple{\denote{\ctx}\wedge\denote{\heap}}
          {\conc{x}}
{\denote{{\tybind{y}{\ty_y}};\ctx} \wedge \denote{\hplocty{\loc}{\tybind{y'}{\ty_{y'}}} \hpjoin \heap'}}
}
\]
\caption{Translation of \rtconc}
\end{figure*}
% $$
% \inference{
%   \hastype{\ctx,\heap}{x}{\tref{\loc}} \quad
%   \iswellformed{\ctx}{\heap = \hplocty{\loc}{\tybind{y}{\ty_y}} \hpjoin \heap'} \\
%   \ty_y = \reft \quad \ty_{y'} = \reftp{\tbase}{\vv = y} \quad y'\;\mbox{fresh}\\
% }{
%   \stmttype
%    {\ctx}
%    {\heap}
%    {\conc{x}}
%    {\ctx;{\tybind{y}{\ty_y}}}
%    {\hplocty{\loc}{\tybind{y'}{\ty_{y'}}} \hpjoin \heap'}
% }[\rtconc]
% $$
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End: 


==> check.tex <==
\section{Type Checking}\label{sec:check}

In this section, we describe how type \emph{checking} works, assuming the
source has been elaborated with heap annotations (\eg
@fold@ and @unfold@) and function signatures.  In
\S~\ref{sec:infer}, we explain how to infer the annotations and
refinement types.

%%%% NUKE NOT ADDING MUCH First, we describe the key judgments of our system, and show how, the 
%%%% NUKE NOT ADDING MUCH typing rules use the heap annotations to precisely track the shape of 
%%%% NUKE NOT ADDING MUCH the heap and updates to heap cells.
%%%% NUKE NOT ADDING MUCH %
%%%% NUKE NOT ADDING MUCH %% Beyond reasoning about the concrete values stored on the heap, \lang's 
%%%% NUKE NOT ADDING MUCH %% type system permits a class of computations, \emph{measures} which 
%%%% NUKE NOT ADDING MUCH %% describe aggregate properties of the structures, to be used in 
%%%% NUKE NOT ADDING MUCH %% refinements.
%%%% NUKE NOT ADDING MUCH %
%%%% NUKE NOT ADDING MUCH Next, we formalize how our system uses the heap annotations 
%%%% NUKE NOT ADDING MUCH to \emph{automatically} strengthen typing environments with 
%%%% NUKE NOT ADDING MUCH \emph{measures} which instantiations, leading to the fully 
%%%% NUKE NOT ADDING MUCH automatic checking of aggregate structure properties like 
%%%% NUKE NOT ADDING MUCH lengths and heights.
%%%% NUKE NOT ADDING MUCH %
%%%% NUKE NOT ADDING MUCH Finally, we outline our strategy for proving the soundness 
%%%% NUKE NOT ADDING MUCH of alias refinement types by translating type rules to 
%%%% NUKE NOT ADDING MUCH separation logic triples.


\subsection{Judgments}

\input{judge}

\mypara{Judgments} The static type system is made of three 
kinds of judgments: \emph{well-formedness} judgments, which
ensure that the refinements only refer to values that are in 
scope at the corresponding program location, \emph{subtyping}
judgments that describe how one set of values or heaps is subsumed
by another, and \emph{typing} judgments that describe the set of 
values and worlds that the evaluation yields.

\mypara{Environments}
%
Our type rules use two kinds of environments:
%
\emph{local} environments, $\ctx$, and \emph{global} environments, $\Phi$. 
%
Local environments are sequences of \emph{type bindings}
$\tb{\evar}{\ty}$ and \emph{guard expressions} $e$.
%
Global environments map functions to their schemas $\tb{\fun}{\funschema}$.
%
We assume that no name is bound twice in an environment.

\mypara{Well-Formedness}
%
We require that types \ty be \emph{well formed} in their
local environments $\ctx$ and heaps $\heap$, written
$\iswellformed{\ctx,\heap}{\ty}$. 
%
A heap $\heap$ must heap be well formed in its local environment
$\ctx$, written $\iswellformed{\ctx}{\heap}$.
%
The rules for the judgment~(\cref{sec:appendixwf})
capture the intuition that a type may only refer to 
binders in its environment.

\mypara{Subtyping}
%
We require a notion of subsumption, \eg 
so that the integer $2$ can be typed either as \reftp{\tint}{\vv=2} 
or simply \tint.
%
The subtyping relation may only 
hold in a given environment. For example, \reftp{\tint}{\vv=x} 
is a subtype of \tnat if \tb{x}{\tnat} holds as well.
%
Subtyping is formalized by the judgment 
$\issubtype{\ctx}{}{\ty_1}{\ty_2}$, whose rules are 
shown in \cref{fig:subtyping}. 
%
Subtyping in \lang reduces to the validity of 
logical implications between refinement predicates.
%
As the refinements are drawn from a decidable logic of Equality, 
Linear Arithmetic, and Uninterpreted Functions, validity
can be automatically checked by SMT solvers \cite{simplifyj}.
%
Type applications are subtyped \emph{covariantly}; as 
updates are handled via the heap, records are essentially pure tuples.
%
The last two rules convert between non-null 
and possibly null references (\tref{\loc} and \trefm{\loc}).
%% Unions of references $\tref{\loc}$ and $\tnull$ types 
%% are subtypes if the corresponding parts are subtypes, 
%% strengthened with the refinement of the union itself.


\mypara{Heap Subtyping} 
%
The heap subtyping judgment $\heapst{\ctx}{\heap}{\heap'}$ describes
when one heap is subsumed by another.
%
\Cref{fig:heapsubtyping} summarizes the rules for heap subsumption.
%
Heap subtyping is \emph{covariant},
which is sound because our type system is flow sensitive --
types in the heap are updated \emph{after} executing a 
statement.

%%%% \mypara{References}
%%%% %
%%%% In \lang, $null$ references and non-$null$ references are given
%%%% different \emph{base} types.
%%%% %
%%%% The judgements \rtref and \rtnull allow expressions to be 
%%%% %
%%%% To represent possibly-$null$ references we use a \emph{union}
%%%% of these two base types.
%%%% %
%%%% Conversion between possibly-$null$ references and the atomic
%%%% non-$null$ (or $null$) references is completely handled via subtyping,
%%%% as discussed earlier. 
%%%% %
%%%% A union may be freely \emph{upcasted} by conjoining the 
%%%% ``missing'' type with the $false$ refinement.
%%%% %
%%%% Dually, a union may be \emph{downcasted} only if the 
%%%% discarded type has the $false$ refinement.
\subsection{Typing}

\mypara{Expressions} 
The judgment {\exprtype{\ctx}{\heap}{\expr}{\ty}}
states that the expression \expr has a type 
\ty in the environment $\ctx$.
%
The typing rules are standard \cite{Knowles10} 
and deferred to \cref{sec:appendixexpr}.

\mypara{Statements}
%
The judgment $\stmttype{\ctx}{\heap}{\stmt}{\ctx'}{\heap'}$ states
that \stmt transforms the environment $\ctx$ and heap \heap into
$\ctx'$ and $\heap'$, respectively.
%
When the condition $x,y$ $\mathit{fresh}$ appears in the antecedent of a rule,
it means that $x$ and $y$ are distinct names that do not appear
in the input environment $\ctx$ or heap $\heap$.
%
We write $\sub{x}{y}$ for the capture avoiding substitution that maps
$x$ to $y$.
%
The rules for sequencing \rtseq, assignment \rtassgn are
straightforward, with \rtassgn adding a new binder
to its output environment.
%
The rule \rtite \emph{joins} the output environment 
and heap of both branches with a super-type. 
%
%% Thus, we treat heaps flow sensitively, and use fresh names to bind
%% heap types as they are updated, which lets us soundly refer to
%% aggregate properties of heap collections (\eg length) as
%% the names are effectively immutable snapshots of structures at a point
%% in time.

\mypara{Allocation}
% 
In \rtalloc, a record is constructed from a sequence of 
field name and expression bindings.
%
The rule types each expression $e_\field$ as $\ty_\field$,
generates a record type $\ty$, and allocates a fresh 
location $\loc$ on the heap whose type is $\ty$. 
%
To connect fields with their containing records, we 
create a new binder $y$ denoting the record, and use 
the helper \fn{NameFields} (\cref{sec:annotstatement}) 
to \emph{strengthen} the type of each field-binding 
for $y$ from 
$\tybind{\field}{\reftpv{\vv_{\field}}{\tbase}{\pred}}$,
to
$\tybind{\field}{\reftpv{\vv_{\field}}{\tbase}{\pred\wedge\vv_{\field} = \fn{Field}(\vv,\field)}}$.
% %TMI
% (Here, \fn{Field} is the \emph{select} operator from SMT decidable 
% theory of arrays\cite{Mccarthy}.)

\mypara{Access}
\rtaccess and \rtmutate both require that \nnull pointers are used
to access a field in a record stored on the heap.
%
As \rtalloc strengthens each type with \fn{NameFields}, the type 
for $y$ in \rtaccess contains the predicate 
$\vv_{f_i} = \fn{Field}(\vv, f_i)$.
%
Any facts established for $y$ are linked, in the refinement logic,
with the original record's field:
when a record field is \emph{mutated}, 
a \emph{new} type binding is created in the heap, and
each unmutated field is 
linked to the old record using $\fn{Field}$.
%

\mypara{Padding}
The statements in either branch of a conditional may allocate 
differing numbers of locations.
%
In order to \emph{join} heaps with different domains, \rtpad
extends the heap with a new location binding, provided that
the new location does not appear in $\ctx$ or $\heap$.
%
This is consistent with our interpretation of heap bindings as
denoting zero or one concrete runtime values.

\mypara{Concretization.}
As heaps also contain bindings of names to types, it would be
tempting to add these bindings to the \emph{local} environment to
strengthen the subtyping context.
%
However, due to the presence of possibly null references, 
adding these bindings would be unsound. Consider the program fragment:
%
\begin{src}
  function f(){ return null; }  ...; p = f(); assert(false); ... 
\end{src}
%
One possible type for @f@ is 
$
\funty{}{\hpemp}{\equant{\loc}\tb{r}{\trefm{\loc}}}{\hplocty{\loc}{\evar}{\reftp{\tint}{\tfalse}}}
$
because the location $\loc$ is unreachable.
%
If we added the binding $\tybind{\evar}{\reftp{\tint}{\tfalse}}$ 
to $\ctx$ after the call to \code{f}, then the subsequent
@assert(false)@ would unsoundly typecheck!

We thus require that in order to include a heap binder in a local
context, $\ctx$, the location must first be made \emph{concrete}, 
by checking that a reference to it is definitely \emph{not} null.
%
Concretization of a location $\loc$ is achieved with the 
\emph{heap annotation} $\concName(x)$.
%
Given a non-null reference, \rtconc transforms the 
local context $\ctx$ and the heap $\heap$ by
(1)~adding the binding $\tybind{y}{\ty_y}$ at the location $\loc$ to
  $\ctx$;
(2)~adding a \emph{fresh} binding $\tybind{z}{\ty_{z}}$ at $\loc$ that
 expresses the equality $y = z$.

%%% Reconsidering @foo@, we note that the reason why $\evar$
%%% receives the $false$ refinement is that the location $\loc$ is
%%% unreachable -- which is only possible because @foo@ is
%%% permitted to return \vnull in lieu of a reference.
%%% %
%%% If, instead, @foo@ were guaranteed to return a reference to
%%% $\loc$, then we could immediately add $\evar$ to $\ctx$ -- 
%%% as the rules for allocation and mutation would preclude 
%%% the \emph{false} refinement from being applied to $\evar$.
%%% %
%%% Concretizations of locations for which there exists a $\nnull$
%%% reference in the local context are thus done automatically at key
%%% points by the type system.

 \mypara{Function Calls and Returns} \rtfuncall uses the parameters to
 carve out the footprint of the caller's heap that is passed to the
 callee, checks the \emph{actual} values and heaps passed in are a
 subtype of those \emph{expected} by the callee, and then uses the
 output heap of the callee to add new locations and update the
 footprint of the caller as needed via the helper \addHeapName.
 \rtreturn checks that the output value and heap are subtypes of the
 expected ones in the given context.

\mypara{Unfold}
%
\rtunwind describes how a type constructor application
$\tyapp{\tycon}{\tvar}$ may be unfolded according to its definition.
%
The context is modified to contain the new heap locations corresponding
to those mentioned in the type's definition.
%
The rule assumes an $\alpha$-renaming such that the locations and binders
appearing in the definition of $\tycon$ are \emph{fresh}, and then instantiates
the formal type variables $\many\tvar$ with the actual $\many\ty$.

\mypara{Fold}
%
Folding a set of heap bindings \emph{into} a
data structure is performed by \rtwind.
%
Intuitively, to fold a heap into a type application of \tycon, we
ensure that it is consistent with the definition of \tycon.
%
Note that the rules assume an appropriate $\alpha$-renaming of the
definition of \tycon.
%
Simply requiring that the heap-to-be-folded be a
subtype of the definition's heap is too restrictive.  Consider the
first @fold@ in @absL@ in \cref{fig:ex3}.
%
As we have reached the end of the list \isnull{xn} we need to fold
$$    
      \hb{\x}{\tb{x_1}{\tobj{\fld{data}{\tnat},\fld{next}{\trefm{\addr{t}}}}}} 
\hsep \hb{t}{\tb{t_0}{\tlist{\tint}}}
$$
into $\hb{\x}{\tb{x_2}{\tlist{\tnat}}}$. 
%
An application of heap subtyping, 
\ie requiring that the heap-to-be-folded is 
a subtype of the body of the type definition,
would require that
%
$\hb{t}{\tlist{\tint}} \relst \hb{t}{\tlist{\tnat}}$,
% \label{eq:intnatlist}
%
which does not hold!
%
However, the fold \emph{is} safe, as  
the @next@ field is \vnull, rendering \addr{t} unreachable.
%
We observe that it is safe to fold a heap into another heap, so long
as the sub-heap of the former that is \emph{reachable from a given
  type} is subsumed by the latter heap.
 
Our intuition is formalized by the relation
$\heapfold{\ctx,\heap}{\ty_1}{\heap_1}{\ty_2}{\heap_2}{x}$, 
which is read: ``given a local context $\ctx, \heap$, 
the type $\ty_1$ and the heap $\heap_1$ may be folded
into the type $\ty_2$ and heap $\heap_2$.''
%
$\rstfoldty{base}$ defines the ordinary case:
from the point of view of a type $\ty$, any heap $\heap_1$ 
may be folded into another heap $\heap_2$.
%
On the other hand, if $\ty_1$ is a reference to a location
$\loc$, then $\rstfoldty{ref}$ additionally requires the 
folding relation to hold at the type bound at $\loc$ in $\heap_1$.

$\rstfoldty{?ref}$ splits into two cases, depending on whether
the reference is null or not.
%
The relation is checked in two strengthened 
environments, respectively assuming the reference is in fact 
null and non-null.
%
This strengthening allows the subtyping judgement to make 
use reachability. Recall the first fold in @absL@ that 
happens when \isnull{\pvar{xn}}. To check the @fold(&x)@, the 
rule requires that the problematic heap subtyping 
%
$\ctx \vdash \hb{t}{\tlist{\tint}} \relst \hb{t}{\tlist{\tnat}}$
%
only holds when $\mathtt{x.next}$ is non-null, \ie when $\ctx$ is
%
$$\tb{\pvar{xn}}{\reftp{\trefm{\addr{t}}}{\vv = \pfield{x_2}{next}}},\ 
  \isnull{\pvar{xn}},\ 
  \isnonnull{\pfield{x_2}{next}}$$
%
This heap subtyping reduces to checking the validity of the following, 
which holds as the antecedent is inconsistent:
$${\pvar{xn}} = \pfield{x_2}{next} \wedge \isnull{\pvar{xn}} \wedge \isnonnull{\pfield{x_2}{next}}
\Rightarrow 0 \leq \vv.$$
%%% \mypara{Calls and Returns}
%%% The rules \rtfun and \rtfuncall modify their output environments
%%% by calling \addHeapName, which greedily checks for locations $\loc$ and
%%% variables $\evar$ such that $\tybind{\evar}{\tref{\loc}} \in \ctx$.
%%% %
%%% If such an $\evar$ exists, the location can be concretized and added
%%% to $\ctx$.
%%% The \lstinline{if} statement checks if \lstinline{xn} is $null$.
%%% %
%%% In the ``then'' branch, the function simply returns, without
%%% updating the type of \lstinline{&xn}.
%%% %
%%% To type check the \windName call, the following subtyping checks
%%% are made to satisfy the folding relation:
%%% \begin{align*}
%%% & \issubtype{\ctx}{}{\reftp{\tnull}{\vv = x_2.\mathtt{next}}}
%%%                     {\tnull}
%%% \\ 
%%% & \issubtype{\ctx}{}{\reftp{\tref{\&t}}{\vv = x_2.\mathtt{next}}}
%%%                     {\tref{\&t}}
%%% \\
%%% &\issubtype{\tybind{z}{\reftp{\tref{\&t}}{\vv = x_2.\mathtt{next} \wedge \vv \neq \vnull}};\ctx}{}
%%%           {\tyapp{\fn{List}}{\tint}}
%%%           {\tyapp{\fn{List}}{nat}}
%%% \end{align*}
%%% %
%%% The first two checks correspond to the subtyping obligations in
%%% \rstfoldty{base} and \rstfoldty{ref}, respectively.
%%% %
%%% The last check is due to the recursive 
%%%   $\heapfold{\ctx}{\heap}{\ty}{\heap_a}{\ty'}{\heap_b}$
%%%   obligation in \rstfoldty{ref}.
%%% %
%%% At first, it seems this check is doomed to failure because
%%% $\tint \not\relst nat$.
%%% %
%%% However, the crucial fact that $x_2.\mathtt{next} = \vnull$
%%% was recorded in $\ctx$ by \rtite.
%%% %
%%% To show that $\reftp{\int}{p} \relst nat$ requires
%%% \[
%%% \validimp{\ctx}{p}{\vv \ge 0}
%%% \]
%%% which, in general, is not true.
%%% %
%%% The contradiction allows the subtyping check to succeed.
%%% %
%%% This is because the subtyping check reduces to the checking the
%%% validity of the formula
%%% \[
%%% z = x_2.\mathtt{next}\wedge{z = \vnull}\wedge{x_2.\mathtt{next} \neq
%%%   \vnull}\wedge\denote{\ctx} \Rightarrow (\vv \ge 0)
%%% \]

%%% Finally, $\rstfoldty{heap}$ defines how record types may be folded.

\subsection{Measures}\label{sec:measures}

%%% NUKED-IN MAIN SYNTAX \begin{figure}
%%% NUKED-IN MAIN SYNTAX   \[
%%% NUKED-IN MAIN SYNTAX    \expr ::=   v                           
%%% NUKED-IN MAIN SYNTAX                \spmid \fn{f}(e)                 
%%% NUKED-IN MAIN SYNTAX                \spmid \expr \op \expr          
%%% NUKED-IN MAIN SYNTAX                \spmid \ite{\evar}{\expr}{\expr}
%%% NUKED-IN MAIN SYNTAX                \spmid \nnite{x.f}{\expr}{\expr}
%%% NUKED-IN MAIN SYNTAX   \]
%%% NUKED-IN MAIN SYNTAX    \caption{Syntax of Measure Expressions}
%%% NUKED-IN MAIN SYNTAX    \label{fig:measuresyntax}
%%% NUKED-IN MAIN SYNTAX \end{figure}

% \input{measurejudge}

Many properties of recursively-defined 
data structures, such as the length of a list or 
the set of keys in a binary search tree, are best 
defined as recursive functions that we call measures.
%
We define measures over \emph{snapshots}, pure values that correspond
to the reachable elements of a data structure.

\mypara{Well-formedness}
Allowing arbitrary recursive functions to appear in 
type refinements would be problematic -- including 
nonterminating computations in types leads to 
unsoundness.
%
Similar concerns about consistency arise
when allowing refinements to refer to values in 
unreachable heap locations.
%
Thus, we require \emph{well-formedness} for measures.
%
Measures must be well defined over
\emph{pure} snapshots,
ensuring that computations over possibly-null
references (\eg the \code{next} field of a \tlist{A}), 
are well defined when the reference is \vnull.

% A measure expression containing a heap binder is well-formed 
% only if a \emph{reference} to that location is tested with 
% a non-null conditional construct \nnite{\code{p}}{\code{m}}{\code{n}} 
% that tests to see if \code{p} is non-$null$.
% %
% If so, then \code{m} is evaluated as the value of the expression.
% %
% Otherwise, \code{n} is evaluated as the value of the non-null conditional.
%
%% Semantically this is equivalent to \ite{\code{p = null}}{\code{m}}{\code{n}}, but provides a syntactic means of
%% guaranteeing that measures are well formed with respect to the heap.

Well-fordmedness 
$\iswellformedMeas{\tyapp{\tycon}{\many\tvar}}{\fn{m}(x) \doteq e}$ (\cref{sec:appendixwf})
restricts the variables that are in the scope of the measure's
body, enforcing well-foundedness and sound heap access.
%
A measure on $\tycon$ is well-formed if it only
references fields of $\tycon$ and is defined on both \vnull and
$\tycon$.
%
Recalling the example from \cref{sec:snapshots},
%
we expand $\fn{len}(v_1)$
\[
\fn{len}(v_0) = 1 + \fn{len}(v_1) = 1 + (1 + \fn{len}(\vnull)) = 1 + (1 + 0) = 2
\]

%
% The definition of \fn{len} over \tlist{\tvar} snapshots
% is thus defined: 
% %
% \[
% \fn{len}(\vnull) = 0\quad
% \fn{len}(x) = 1 + \fn{len}(x.next)
% \]
% %
% where $\pi_2$ is the usual second projection -- used in this case
% to access the snapshot of the next list node.

\mypara{Instantiation}
%
Unfolding yields records that are \emph{assumed} to 
satisfy the invariants of the aggregate structure,
%
while folding \emph{checks} that individual 
locations satisfy the structure invariants.
%
These operations are convenient for instantiating
the facts encapsulated by measures.

% \mypara{Unfolding Instantiates, Fold Generalizes}
% Unfolding yields records that are \emph{assumed} to 
% satisfy the invariants of the aggregate structure. 
% For example, a $\tlist{\tnat}$ is unfolded into a head record
% whose @data@ field can be assumed to be a \tnat.
% Thus, unfolding is a robust syntactic means of 
% \emph{instantiating} universal facts about the 
% structure.
% %
% Dually, folding \emph{checks} that individual 
% locations satisfy the invariants of the aggregate structure.
% For example, in @absL@ we fold a single head 
% cell that has a \tnat @data@ field, and a \tlist{\tnat} 
% into a single \tlist{\tnat}.
% Thus, folding is a robust syntactic means of \emph{generalizing}
% universal facts from specific locations.
% %
% We will use exactly the same idea to automatically 
% reason about global properties defined by measures 
% (\eg lengths) and abstract refinement (\eg ordering).

% corresponds to the asertion of (1) an uninterpreted predicate
% corresponding to the \emph{base} type of $\evar$ and (2) its refinement.
% %
% Thus, if ${\ctx} = \tybind{\evar}{\reftp{\tint}{\vv > 0}}$, then 
% $\denote{\ctx} = \suif{int}(x)\wedge(x > 0)$.
% %
% Interpretations of type judgements are given in
% \cref{fig:interp-judge}.
% %
%%%% {{{ 
%%%% Our system includes a set of heap manipulating annotations that
%%%% transform the \emph{shape} of the heap, by which we mean the set of mapped locations
%%%% and the refined types at mapped at those locations.
%%%% %
%%%% The annotations, which may be thought of as program statements with
%%%% no observable effect, direct the type system to precisely track
%%%% updates to the types of values stored in collections.
%%%% %
%%%% We automatically infer locations for these annotations in order to reduce
%%%% the burden on the programmer.
%%%% %
%%%% Beyond reasoning about the concrete values stored on the
%%%% heap, the type system permits a class of
%%%% computations, \emph{measures}, to be used in refinements.
%%%% %
%%%% These computations may be used to define properties such as the length
%%%% of a list or the height of a tree, and are \emph{automatically}
%%%% instantiated by the type system.
%%%% 
%%%% In the remainder we first introduce and discuss the typing judgements
%%%% for alias refinement types.
%%%% %
%%%% We then describe measures, and how they may be soundly added to the type system.
%%%% %
%%%% Next, we give the algorithm \toolname, our implementation of alias
%%%% refinement types, uses to infer annotation locations.
%%%% %
%%%% Finally, we outline our strategy for proving the soundness of alias
%%%% refinement types by translating type rules to separation logic
%%%% triples.
%%%%% Alias refinement types are based on liquid types, a refinement type
%%%%% system that has been used to reason about heap manipulating,
%%%%% imperative code.
%%%%% %
%%%%% As in \liquid, a type $\reft$ is a base type, $\tbase$, together with a
%%%%% predicate, $\pred$.
%%%%% %
%%%%% The type \reft describes all \vv of type \tbase where \pred is true.
%%%%% %
%%%%% The remainder of this section describes our type system for concluding
%%%%% that expressions and statements are well-typed.
%%%% }}}


%%% Local Variables: 
%%% mode: latex
%%% eval: (TeX-PDF-mode 1)
%%% TeX-master: "main.tex"
%%% End: 


==> commands.tex <==
%%%%%%%%%%% English %%%%%%%%%%%%
\newcommand\etc{\textit{etc.}\xspace}
\newcommand\eg{\textit{e.g.}\xspace}

\def\emphbf#1{\textbf{\emph{#1}}}
\def\myexsh{\smallskip\noindent{\emphbf{Example.}\xspace}}
% \def\myex#1{\smallskip\noindent{\emphbf{Example: {#1}.}}}
\newcommand\spara[1]{\smallskip\noindent\textbf{\emph{#1}}\xspace}
\newcommand\mypara[1]{\spara{#1}}
%\def\mypara#1{\smallskip\noindent\textbf{#1.}\ }


%%%%%%%%%%% Maths    %%%%%%%%%%%
\newcommand\many{\overline}
\def\colon{\ensuremath{\text{:}}}

\newcommand{\relDescription}[1]{\ensuremath{\textrm{\textbf{#1}}}}
\newcommand{\judgementHead}[2]{\ensuremath{\relDescription{#1}\hfill\fbox{#2}}}
\newcommand{\judgementHeadNameOnly}[1]{\ensuremath{\relDescription{#1}\hfill}}

\newenvironment{sitemize}{\begin{list}
   {$\bullet$}
   {\setlength{\topsep}{0pt}
    \setlength{\itemsep}{0pt}
    \setlength{\leftmargin}{15pt}
    }
  }
  {\end{list}}

\newcommand{\code}[1]{\texttt{#1}}
%%%%%%%%%%% Language %%%%%%%%%%%
\newcommand{\lang}{\ensuremath{LImp}\xspace}

\newcommand\spmid{\ \mid \ }
\newcommand\op{\ensuremath{\oplus}\xspace}

\newcommand\field{f\xspace}
% Values
\newcommand\val{\ensuremath{v}\xspace}
\newcommand\vnum{\ensuremath{n}\xspace}
\newcommand\vref{\ensuremath{r}\xspace}

% Expressions
\newcommand\expr{\ensuremath{e}\xspace}
\newcommand\evar{\ensuremath{x}\xspace}
\newcommand{\funcall}[1]{\ensuremath{f(#1)}\xspace}
\newcommand{\access}[2]{#1.#2}

% Statements
\newcommand\stmt{\ensuremath{s}\xspace}
\newcommand{\unwind}[1]{\code{unwind}(#1)\xspace}
\newcommand{\wind}[2]{\code{wind}(#1 \leadsto #2)\xspace}
\newcommand{\rename}[2]{\code{rename}(#1 \mapsto #2)\xspace}
\newcommand{\return}[1]{\code{return}\; #1\xspace}
\newcommand{\ite}[3]{\code{if}\;#1\;\code{then}\;#2\;\code{else}\;#3\xspace}
\newcommand{\alloc}[1]{\code{alloc}\;\{#1\}\xspace}

%% Types
\newcommand\loc{\ensuremath{l}\xspace}
\newcommand\localt{\ensuremath{m}\xspace}
\newcommand\tycon{\ensuremath{C}\xspace}
\newcommand\tbase{\ensuremath{b}\xspace}
\newcommand\tint{\ensuremath{int}\xspace}
\newcommand\tvar{\ensuremath{\alpha}\xspace}
\newcommand{\tref}[1]{\ensuremath{ref(#1)}\xspace}
\newcommand{\tobj}[1]{\ensuremath{\{#1\}}\xspace}
\newcommand{\tyapp}[2]{\ensuremath{#1[#2]}\xspace}

%% RefTypes
\newcommand\ty{\ensuremath{\tau}\xspace}
\newcommand{\reft}{\ensuremath{\{\vv : \tbase \,\mid\,\pred \}}\xspace}
\newcommand{\pred}{\ensuremath{p}\xspace}
\newcommand{\vv}{\ensuremath{\nu}\xspace}

%% Heaps
\newcommand{\heap}{\ensuremath{\Sigma}\xspace}
\newcommand{\hplocty}[2]{\ensuremath{#1 \mapsto #2}}
\newcommand{\hpemp}{\ensuremath{emp}\xspace}
\newcommand{\hpjoin}{\ensuremath{\ast}\xspace}

\newcommand{\vartybind}{\ensuremath{\evar:\ty}}

%%Functions
\newcommand{\funschema}{\ensuremath{S}\xspace}
\newcommand{\funty}[4]{\ensuremath{(#1)/#2 \rightarrow #3/#4}\xspace}
\newcommand{\fundecl}[2]{\texttt{function}\;#1(#2)\;
                            \texttt{\{}\stmt\texttt{\}}\xspace}
\newcommand{\fun}{\ensuremath{f}\xspace}

%%Forall
\newcommand{\quant}[1]{\ensuremath{\forall{#1}.}\;\xspace}

%%Programs
\newcommand{\prog}{\ensuremath{p}\xspace}

%%TyDefs
\newcommand{\tydef}[4]{\ensuremath{\code{type}\;#1=\uniqex{#2}#3:#4\xspace}}

\newcommand{\uniqex}[1]{\ensuremath{\exists{!\;#1}.\;\xspace}}

%%Hoare Rules
%% \newcommand{\htriple}[3]{\ensuremath{\{\;#1\;\}}\;#2\;\ensuremath{\{\;#3\;\}}\xspace}
\newcommand{\htriple}{foo}
%% \newcommand{\htriplec}[3]{\htriple{#1}{\code{#2}}{#3\}}}


==> conclusion.tex <==
\section{Conclusions and Future Work}\label{sec:conclusion}
\abakst{new}
In this paper, we have shown through \toolname that decoupling the
shape of data structures from their logical properties admits an
effective, syntax-directed method for verifying and inferring precise
invariants of data structures.
%
We have shown that \toolname identifies a fragment of separation
logic that is both automatic \emph{and} expressive.
%
As such, possible future work includes extending \toolname with
SL-based techniques to support concurrency, improve automation, 
and handle more sophisticated data structures.
%
%
% That is, \toolname identifies a fragment of SL which is the 
% composition of two sub-logics, namely: alias-typing for 
% the heap, and refinement-typing for the data.
% %
% ``Physical" alias-typing allows us to update 
% the heap \emph{locally} at writes, \emph{folds} or \emph{unfolds}, 
% relieving the ``logical" refinement system of the burden 
% of reasoning about aliasing or reachability.
% %
% By composing the logics and their respective decision procedures 
% -- alias typing for the heap, and refinement/liquid typing for the data --
% \toolname identifies a fragment of SL that is automatic \emph{and} expressive.
% %
% Currently \toolname is limited to structures describable via alias 
% types. We have shown experimentally that it is rich enough to include 
% doubly- and circularly linked lists and various complex trees.
% %
% As \toolname is a stylized fragment of separation logic with a 
% syntax directed decision procedure, avenues for future work include
% extending it directly with SL based techniques to support 
% more structures, or improve efficiency and automation.

%%% In this paper we have described a solution to the problem of
%%% verifying properties of linked data structures.
%%% %
%%% Our approach, \emph{Alias Refinement Types} (\toolname), leverage
%%% Alias Types and Refinement Types to enable the inference
%%% of semantic properties of data structures.
%%% %
%%% We have implemented \toolname and evaluated it on a number of
%%% well-known data structures in order to verify implementations of
%%% sorted lists and red-black trees.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End: 


==> examples/ex12.tex <==
\rowcolors{2}{gray!5}{}
\begin{figure}[ht!]
  \begin{minipage}[ht!]{0.5\textwidth}
  \begin{center}
% @  //: abs :: (int) => nat@\\
  \ra{0.8}
\begin{tabular}{|ll|}
  \hline
  \multicolumn{2}{|c|}{\sfunty{abs}{\tint}{\tnat}}\\
  \hline
  \hline
@function abs(x){@  & \spmid \tb{\x}{\tint}                 \\ 
@  if (0 <= x)   @  & \spmid \quad \same\ ,\ \grd{(0 \leq \x)} \\ 
@    return x;   @  & \spmid \\
@  var r = 0 - x;@  & \spmid \same\ ,\ \grd{\lnot(0 \leq \x)},\ \tb{\pvar{r}}{\refp{\vv = 0 - \x}} \\
@  return r;     @  & \spmid \\
@} @                & \\
\hline
\end{tabular}
\captionof{figure}{Refinement Types}\label{fig:ex1}
\end{center}
\end{minipage}
\begin{minipage}[ht!]{0.5\textwidth}
% @// absR :: (x:{data:int}) => void/&x |->{data:nat}@\\
\setlength{\tabcolsep}{0.15em}
\ra{0.9}
\begin{tabular}{|lll|}
\hline
\multicolumn{3}{|c|}{\sfunty{absR}
                            {\tb{\x}{\tobj{\fld{data}{\tint}}}}   
                            {\tvoid/\hb{x}{\tobj{\fld{data}{\tnat}}}}} \\
\hline
\hline
@function absR(x){@   & \spmid \tb{\x}{\tref{\addr{\x}}}                 & \esep $\hb{\x}{\tobj{\fld{data}{\tint}}}$ \\ 
@  var d  = x.data;@  & \spmid \same\ ,\ \tb{\pvar{d}}{\tint} & \esep \same \\ 
@  var t  = abs(d);@  & \spmid \same\ ,\ \tb{\pvar{t}}{\tnat} & \esep \same  \\
@  x.data = t;@       & \spmid \same                                   & \esep $\hb{\x}{\tobj{\fld{data}{\tnat}}}$\\
@  return;@           & & \\
@}@                   & & \\
\hline
\end{tabular}
\captionof{figure}{Strongly Updating a Single Location}\label{fig:ex2}
\end{minipage}
\end{figure}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../main"
%%% End: 


==> examples/ex3-a.tex <==
% \rowcolors{2}{gray!5}{}
\rowcolors{1}{}{}
\begin{figure*}[t] 
\ra{1.0}
  \begin{center}
\begin{tabular}{|ll|}
  \hline
  \multicolumn{2}{|c|}{\sfunty{absL}
                              {\tb{\x}{\tlist{\tint}}}
                              {\tvoid / \hb{\x}{\tlist{\tnat}}}} \\
  \hline
  \hline
@function absL(x){ @  \cellcolor[gray]{0.9}&
\cellcolor[gray]{0.9}
 $\ctx_0 \doteq \tb{\x}{\tref{\addr{\x}}}$,
 $\heap_0 \doteq  \hb{\x}{\tb{x_0}{\tlist{\tint}}}$
 \\ 
@  //: unfold(&x); @  & \multirow{2}{*}{
  \begin{minipage}{0.7\textwidth}
    $\ctx_1 \doteq \ctx_0$ \\
    $\heap_1 \doteq \hb{\x}{\tb{x_1}{\tobj{\fld{data}{\tint},\fld{next}{\trefm{\addr{t}}}}}} \hsep \hb{t}{\tb{t_0}{\tlist{\tint}}}$
  \end{minipage}
}\\
& \\
@  var d  = x.data;@ \cellcolor[gray]{0.9} & \cellcolor[gray]{0.9} \\
%%\spmid \same\ ,\ \tb{\pvar{d}}{\tint} 
%%\esep \same 
@  x.data = abs(d);@ \cellcolor[gray]{0.9} & \cellcolor[gray]{0.9}
%%\spmid \same 
%%\esep \hb{\x}{\tb{x_2}{\tobj{\fld{data}{\tnat},\fld{next}{\trefm{\addr{t}}}}}}
%%\hsep \hb{t}{\tb{t_0}{\tlist{\tint}}}                          
\\
@  var xn = x.next;@ \cellcolor[gray]{0.9} & \cellcolor[gray]{0.9}\multirow{-3}{*}{
  \begin{minipage}{0.7\textwidth}
    $\ctx_2 \doteq \tb{\pvar{d}}{\tint},\, 
\tb{\pvar{xn}}{\reftp{\trefm{\addr{t}}}{\vv = \pfield{x_2}{next}}},\, \ctx_1$
    \\[-0.02in] 
    $\heap_2 \doteq 
\hb{\x}{\tb{x_2}{\tobj{\fld{data}{\tnat},\fld{next}{\trefm{\addr{t}}}}}}
\hsep \hb{t}{\tb{t_0}{\tlist{\tint}}}$
  \end{minipage}
}
% \spmid \same\ ,\ \tb{\pvar{xn}}{\reftp{\trefm{\addr{t}}}{\vv = \pfield{x_2}{next}}} \esep \same 
\\
@  if (xn == null){@  &  \\
@    //: fold(&x); @\cellcolor[gray]{0.9}   & \cellcolor[gray]{0.9} 
$\ctx_3 \doteq \isnull{\pvar{xn}},\, \ctx_2$, $\heap_3 \doteq\hb{\x}{\tlist{\tnat}} $\\
@    return;       @  & \\
@  }               @  & \\
@  absL(xn);       @\cellcolor[gray]{0.9}  & \cellcolor[gray]{0.9}\\

&\cellcolor[gray]{0.9}\multirow{-2}{*}{
    \begin{minipage}{0.7\textwidth}
      $\ctx_4 \doteq \isnonnull{\pvar{xn}};\ctx_2$\\
      $\heap_4 \doteq \hb{\x}{\tb{x_2}{\tobj{\fld{data}{\tnat},\fld{next}{\trefm{\addr{t}}}}}} \hsep \hb{t}{\tb{t_1}{\tlist{\tnat}}}$
    \end{minipage}
}
\\
@  //: fold(&x);   @  &\cellcolor[gray]{1.0} $\ctx_5 \doteq \ctx_4$ $\heap_5 \doteq \hb{\x}{\tb{x_3}{\tlist{\tnat}}}$ \\ 
@  return;         @  & \\
@}                 @  & \\
\hline
\end{tabular}
\caption{Strongly Updating All Locations Of A Collection}\label{fig:ex3}
\end{center}
\end{figure*}


==> examples/ex5.tex <==
\begin{figure*}[ht]
\ra{0.9}
@ //: iSort :: (x:?list[A]) => {v:?list[A]| len(v)=len(x)}@\\
\begin{tabular}{lll}
& & \\
@function iSort(x) {   @ & \spmid \tb{x}{\tref{\addr{x}}} 
                         & \esep  \hb{x}{\tb{x_0}{\tlist{A}}} \\ 
@  if (x == null)      @ & \spmid \quad \same\ ,\ \isnull{x} 
                         & \same \\
@    return null;      @ & & \\
@  //: unfold(&x);     @ & \spmid \same\ ,\ \mlen{x_0} = 1 + \mlen{t_0} 
                         & \esep \hb{x}{\tb{x_1}{\tobj{\fld{data}{A}, \fld{next}{\trefm{\addr{t}}}}}}
                           \hsep \hb{t}{\tb{t_0}{\tlist{A}}} \\
@  var h = x.data;     @ & \spmid \same\ , \tb{h}{A} 
                         & \same \\
@  var t = x.next;     @ & \spmid \same\ , \tb{t}{\trefm{\addr{t}}} 
                         & \same \\
@  var y = iSort(t);   @ & \spmid \same\ , \tb{y}{\trefm{\addr{y}}}\ ,\ \mlen{y_0} = \mlen{t_0}
                         & \esep \hb{x}{\tb{x_1}{\tobj{\fld{data}{A}, \fld{next}{\trefm{\addr{t}}}}}}
                           \hsep \hb{y}{\tb{y_0}{\tlist{A}}} \\
@  var z = insert(h,y);@ & \spmid \same\ ,\ \tb{z}{\tref{\addr{z}}}, \mlen{z_0} = 1 + \mlen{y_0} 
                         & \esep \hb{x}{\tb{x_1}{\tobj{\fld{data}{A}, \fld{next}{\trefm{\addr{t}}}}}}
                           \hsep \hb{z}{\tb{z_0}{\tlist{A}}} \\
@  return z;           @ & & \\
@}                     @ & & \\
\end{tabular}
\caption{Insertion Sort}\label{fig:ex5}
\end{figure*}


==> examples/ex6.tex <==
\rowcolors{2}{gray!5}{}
\begin{figure*}[ht]
\ra{1.0}
  \begin{center}
%% @  //: insert :: (A, x:?list[A]) => {v:list[A] | len(v) = 1 + len(x)}@ \\
\setlength{\tabcolsep}{0.15em}
\begin{tabular}{|lll|}
  \hline
  \multicolumn{3}{|c|}{\sfunty{insert}
                              {A, \tb{x}{?\tlist{A}}}
                              {\reftp{\tlist{A}}{\mlen{\vv} = 1 + \mlen{x}}}} \\
  \hline
  \hline
@function insert(k, x){ @ & \spmid \tb{k}{A},\ \tb{x}{\tref{\addr{x}}} 
                          & \esep \hb{x}{\tb{x_0}{\tlist{A}}} \\ 
@                       @ & \multicolumn{2}{l|}{$\hookrightarrow 
                            \hassert{\exquant{\loc_x x_0}
                             (x = \loc_x \vee \isnull{x}) 
                             \hpjoin 
                             (\loc_x = null \vee \fn{list}(A, \loc_x, x_0))
                            }$}\\
@  if (x == null) {     @ & \spmid \quad \same\ ,\ \isnull{x} & \esep \\
@                       @ & \multicolumn{2}{l|}{$\hookrightarrow 
                            \hassert{\same \wedge (x = \tnull) \hpjoin \same
                            }$}\\
@    var y  = {};       @ & & \\
@    y.data = k;        @ & & \\
@    y.next = null;     @ & \spmid \quad \same\ ,\ \tb{y}{\tref{\addr{y}}} 
                          & \esep \hb{x}{\tb{x_0}{\tlist{A}}}
                            \hsep \hb{y}{\tb{y_0}{\tobj{\fld{data}{A}, \fld{next}{\tnull}}}} \\ 
@                       @ & \multicolumn{2}{l|}{$\hookrightarrow
                            \hassert{
                              \same\exquant{\loc_y y}
                              (y = \loc_y \wedge \isnonnull{y})
                              \wedge \same 
                              \hpjoin 
                              (\sepmap{\loc_y}{y} 
                                 \wedge 
                                 y = \tobj{\fld{data}
                                               {\objfield{y}{\code{data}}},
                                           \fld{next}
                                               {\tnull}})}
                                           $}\\
@    //: fold(&y)       @ & \spmid \quad \same\ ,\ \mlen{y_1} = 1 
                          & \esep \hb{x}{\tb{x_0}{\tlist{A}}}
                            \hsep \hb{y}{\tb{y_1}{\tlist{A}}} \\
@    return y;          @ & & \\
@  }                    @ & & \\
@  ...                  @ & & \\
@}                      @ & & \\
\hline
\end{tabular}
\caption{Inserting into a Collection}\label{fig:ex6}
\end{center}
\end{figure*}


==> hsubtyping.tex <==
% \begin{lemma}\label{l:heapsubtyping}
% \showheapsubtyping
% \end{lemma}
\begin{proof}
  By induction on the subtyping derivation.
  %
  In each case we remember that since $\loc$ does not appear in $\ctx$, 
  $\denote{\ctx}$ never implies $\loc \neq null$.
  %
  \begin{enumerate}
    \item[\textsc{Case} $\issubtype{\ctx}{}{\hpemp}{\hpemp}$] \hfill \\
      The heaps are equivalent and their domains are empty, so the conclusion is 
      trivially true.
    \item[\textsc{Case} 
      $\issubtype{\ctx}{}{\heap}
                           {\heap\hpjoin\hplocty{\loc}{\evar}{\ty}}$]
      \hfill \\
      By well-formedness, $\loc \not\in \dom{\heap}$, so the conclusion is
      vacuously true.
    \item[\textsc{Case} 
      $\issubtype{\ctx}{}{\heap\hpjoin\hplocty{\loc}{\evar}{\ty}}
                           {\heap'\hpjoin\hplocty{\loc}{\evar}{\ty'}}$]
      \hfill \\
      By assumption, 
      since for every $\loc' \neq \loc \in \dom{\heap} \cap \dom{\heap'}$, 
      $\issubtype{\ctx}{}{\ty_{\loc'}}{\ty'_{\loc'}}$
      when $\hplocty{\loc'}{y}{\ty_{\loc'}} \in \heap$ and
      $\hplocty{\loc'}{y}{\ty'_{\loc'}} \in \heap'$. 
    \end{enumerate}
    %
    Furthermore, the well-formedness conditions in each rule ensure by
    \cref{l:wfheap} that each singleton location assertion occurs only once.
  \end{proof}
  %%% Local Variables: 
  
% \begin{lemma}\label{l:heapsubtyping2}
\showheapsubtypingdos
% \end{lemma}
\begin{proof}
%
By \cref{l:heapsubtyping}, for each $\loc \in \dom{\heap_1} \cap
\dom{\heap_2}$, when $\hplocty{\loc}{x}{\ty} \in \heap_1$ and
$\hplocty{\loc}{x}{\ty'} \in \heap_2$, then
%
\begin{align*}
  \exquant{\loc\ldots}.
  \denote{\ctx} \Rightarrow \sprop{\ty}{x} \Rightarrow \sprop{\ty'}{x}
\end{align*}
%
and thus, assuming without loss of generality that $\ty$ (and thus $\ty'$) are
are record types,
%
\begin{align*}
  \exquant{\loc\ldots x\ldots}
  \denote{\ctx}
  & \Rightarrow (\sepmap{\loc}{x}\wedge\sprop{\ty}{x}) \\
  & \Rightarrow ((\loc = null) \vee (\sepmap{\loc}{x}\wedge\sprop{\ty'}{x}))
\end{align*}
%
And hence, by definition,
%
\begin{align}
  \exquant{\loc\ldots x\ldots}
  \denote{\ctx}
  & \Rightarrow \denote{\hplocty{\loc}{x}{\ty}} \nonumber \\
  & \Rightarrow \denote{\hplocty{\loc}{x}{\ty'}} \label{fact1}
\end{align}
%
As for each $\loc' \in \heap_2$ that does not appear in $\ctx$ or $\heap_1$, we may
conclude
%
\begin{align*}
  \exquant{\loc'}\loc' = null \label{fact2}
\end{align*}
%
Therefore, for each $\loc \in \dom{\heap_1} \cap \dom{\heap_2} \cup \locs{\ctx}$,
%
\begin{equation}
\exquant{\loc x}.
\denote{\ctx}\wedge\denote{\hplocty{\loc}{x}{\ty}} \Rightarrow \denote{\hplocty{\loc}{x}{\ty'}}
\label{fact2}
\end{equation}
% 
by \cref{fact1}.
%
For each $\loc' \in \dom{\heap_2} \setminus \dom{\heap_1} \cup \locs{\ctx}$
%
\[
\exquant{\loc'}.
\denote{\ctx}
\Rightarrow 
\exquant{\loc'}(\loc' = null) 
\Rightarrow 
\denote{\hplocty{\loc}{x}{\ty'}}
\]
%
by \cref{fact2}.
%
Since $\denote{\heap}$ is a conjunction (via \hpjoin) of these assertions, we conclude
%
\[
\denotef{\ctx}{\heap_1} \Rightarrow \denotef{\ctx}{\heap_2}
\]
% \begin{enumerate}[(i)]
% \item $\loc \in \dom{\heap_1}$ and 
% \end{enumerate}
\end{proof}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "proof_main.tex"
%%% End: 


==> infer.tex <==
\section{Inference} \label{sec:infer}

With \toolname, the user provides (unrefined) 
function type signatures, and the tool 
automatically infers 
%
(1)~heap annotations required for alias typing, and
%
(2)~refinements that capture correctness invariants.
%
%% Given the type ${(?\tlist{A}) \Rightarrow \tlist{A}}$
%% for @insertSort@, \toolname infers the refinement type:
%% $$(\tb{x}{?\tlist{A}}) \Rightarrow \reftp{?\tolist{A}}{\mlen{\vv} = \mlen{x}}$$
%% \ie it returns an ordered list with as many elements as the input.

\subsection{Heap Annotation Inference}
%
\toolname first infers its input is well-(alias)-typed with 
respect to the supplied unrefined types. 
This \emph{``physical"} checking  phase is like the 
refinement type checking with all refinements erased.
%
\toolname maintains an environment, $\ctx$, of local variable type 
information; and a heap, $\heap$, mapping locations to 
(unrefined) types.

Due to the interaction between unrefined types in 
$\ctx$ and $\heap$, \toolname must necessarily perform 
some heap manipulations.
%
As checking proceeds, \toolname decorates its 
input with \concName, 
%\padName, 
\unwindName, and \windName 
annotations, recording the manipulation of 
the heap, \ie the set of locations, and the types 
at each location. 

\mypara{Concretization} 
%
Preceding any read or write of a record,
if the reference through which the access occurs
is possibly null (\ie \trefm{\loc}), the type checker 
inserts a \concName annotation.
Note that the non-null check inserted by the \concName only fails
if the original program could possibly dereference a null pointer.

%% \myexsh.
%% Consider the \code{absRec} function from Section\ref{sec:overview}.
%% Location \code{\&x} in the caller's\abakst{need a better example here}
%% Thus, after each function call, the type checker inserts \concName
%% calls for each location that is syntactically guaranteed to be
%% \nnull.
%% %
%% Early versions of \toolname did not include this case, which required
%% inserting ``dummy reads'' after some function calls.

\mypara{Unfold}
%
During the physical type checking, \toolname checks 
the type stored at each derefenced location.
%
The type system of \lang permits two types of heap 
stored values: records and type applications.
%
If an operation corresponds to a read or write at a
location containing a \emph{type application}, then 
\toolname must \emph{open} the type constructor to 
ensure that the field access is valid.
%
To this end, \toolname places an \unwindName before 
these accesses, recording the unfolded location and its type.

Recall \lstinline{absL} from \S~\ref{sec:overview}.
Prior to the read of @x.data@, the heap contains the binding
$\hb{x}{\tb{x_0}{\tlist{\tint}}}$
which is not a record containing a \fn{data} field.
An unfold of \addr{x}
transforms the heap to 
\[\hb{x}{\tb{x_1}{\tobj{\fld{data}{\tint},\fld{next}{\trefm{\addr{t}}}}}} 
                      \hsep \hb{t}{\tb{t_0}{\tlist{\tint}}}\]
%% \[
%%   \hplocty{\loc'}{tl}{\tyapp{\fn{List}}{\fn{number}}}
%% \]
%%   and a record 
%% \[
%%  \tobj{\tybind{\fn{data}}{\fn{number}}
%%       ,\tybind{\fn{next}}{\tref{\loc'}}}
%% \]
%
Now, the location referred to by @x@ indeed contains a record with a @data@
field, so the access (physically) type checks. 
Hence, \toolname inserts an \unwindName to record 
that it unfolded a $\tlist{\tint}$ at \addr{x}.

\mypara{Fold}
%
At first glance, it may seem that \toolname need only 
insert {\windName}s preceeding \returnName statements.
%
However, conditionals are another obstacle: each of the 
two possible branches of an \code{if} statement may 
manipulate the heap in different ways.
%
To ensure a consistent view of the heap, \toolname folds up any
unfolded location, \loc, that satisfies at least one of the following criteria:
%
\begin{inparaenum}[(1)]
  \item \loc was folded \emph{before} the \code{if} statement; or
  \item updates to references in the type stored at \loc were made 
        inconsistently between the \code{then} and \code{else} branches.
\end{inparaenum}

This syntax-directed method infers 
heap annotations suitable for refinement type 
inference. (For details, see~\cref{sec:annots}.)

\subsection{Refinement Inference}
%
We use the framework of Liquid Typing
~\cite{LiquidPLDI08} to infer refinements. As in \cite{LiquidPLDI08}, we 
interpret \toolname's typing rules as a type inference algorithm, by: 

\begin{inparaenum}[(1)]
%
\item~For each unknown type in the program, we create a new \emph{template},
    which is the physical (unrefined) type inferred by the physical checking, 
    with refinement variables $\kappa$ representing unknown refinements.
    %
\item~Next, we perform refinement type checking with the templates, 
    obtaining subtyping constraints over the templates, which are 
    reduced via the subtyping rules to a set of implication constraints 
    (or Horn clauses) of the form 
    $(p \wedge_i \kappa_i) \Rightarrow (q \wedge_j \kappa_j)$. 
%
\item~Finally, we solve the implication constraints by abstract 
    interpretation, over a predicate abstraction domain generated 
    by a user-specified set of predicate templates.
    Replacing each $\kappa$ variable with its solution yields 
    the inferred types.
\end{inparaenum}

Thanks to \toolname's decoupling of physical and logical reasoning, 
the refinements are heap-oblivious formulas QF-EUFLIA~\cite{simplifyj},
which lets us use off-the-shelf SMT solvers to infer refinements.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End: 


==> interp.tex <==
\begin{figure*}
\begin{align*}
  \denote{\ctx/\heap} & = \exists{FV(\heap).\,dom(\heap)}.\;\denote{\ctx}\wedge\denote{\heap} \\
\denote{\ctx} & = 
\bigwedge\limits_{\tybind{\evar}{\ty} \in \ctx}  \sprop{\ty}{\evar} \wedge
\bigwedge\limits_{\code{type}\dots \in \ctx}  \sepdef{\code{type}\;t = T} \\
\\
\denote{\heap} & = (\underset{\hplocty{\loc}{\tybind{\evar}{\ty}} \in \heap}{\hpjoin}(\loc = null \vee \shprop{\ty}{\loc}{\evar}))
%%%
\end{align*}
%%%
\begin{align*}
\sbase{\tbase}{\evar} & =
 \begin{cases}
   \suif{int}(\evar) & \tbase = \tint \\
   \evar = \loc \wedge \loc \neq null & \tbase = \tref{\loc} \\
   \evar = null & \tbase = \null \\
   \cdots & \cdots\\
  \end{cases}
\\
%%
\sprop{\reft}{\evar} & =
\begin{cases}
 \stapp{\quant{y}\sprop{\ty}{y}}{\evar}
 \wedge \sub{\vv}{\evar}\pred 
   & \tbase = \tyapp{\tycon}{\ty}
  \\
  (\bigwedge\limits_{\tybind{\field_i}{\ty_i}\in b}
    \sprop{\ty_i}{\objfield{\evar}{\field_i}})
   \wedge\sub{\vv}{\evar}\pred
  & \tbase = \tobj{\many{\tybind{\field_i}{\ty_i}}} \\
 % \stbase(\evar) \wedge \sub{\vv}{\evar}\pred 
  \sbase{\tbase}{\evar}\wedge \sub{\vv}{\evar}\pred 
  & otherwise 
\end{cases} 
\\
%%%
\shprop{\reft}{\loc}{\evar} & =
\begin{cases}
  \shtapp{\quant{y}\sprop{\ty}{y}}{\loc}{\evar} \wedge \sub{\vv}{\evar}\pred
   & \tbase = \tyapp{\tycon}{\ty}
  \\
 \sepmap{\loc}{\evar} \wedge \sprop{\reft}{\evar}
   & otherwise 
\end{cases} 
\\
%%%
\sepdef{
    \tydef{\tyapp{\tycon}{\many{\tvar}}}
                         {\heap}
                         {\evar}
                         {\tobj{\many{f:\ty}}}} & = 
(\shtapp{\pred}{\loc}{\evar} \myeq \equant{\textsf{FV(\heap)},\,dom(\heap)}\denote{\heap\hpjoin\hplocty{\loc}{\tybind{\evar}{\tobj{\many{\field:\ty}}}}}) \\
%%%
\end{align*}
\caption{Interpretation of contexts}
\label{fig:interp-types}
\end{figure*}

%%% Local Variables: 
%%% mode: latex
%%% eval: (TeX-PDF-mode 1)
%%% TeX-master: "main.tex"
%%% End: 


==> intro.tex <==
\section{Introduction}\label{sec:intro}

We present a novel type-based approach to the 
long standing problem of algorithmic verification 
of functional correctness properties of linked 
data structures.
%
The main challenge with verifying linked structures 
is to precisely reason about relationships between
an \emph{unbounded} number of heap locations. 
%
%This requires ways to \emph{generalize} invariants
%over a few locations into a summary describing the 
%entire structure, and, dually, ways to \emph{instantiate} 
%the summary to obtain properties of particular locations.

Previous efforts at algorithmically verifying linked 
structures fall, roughly speaking, into two categories. 
%
The first class of approaches use special \emph{logics} 
that encode unboundedness via special forms of quantification 
and transitive closure \cite{LahiriQadeer08} or with
recursively defined predicates describing the heap 
\cite{BI01,ChinDNQ12,Qiu0SM13}.
%
While these logical approaches are expressive enough 
to be be extensible to a variety of structures and 
properties, they require specialized decision procedures 
which preclude the automated \emph{inference} of 
invariants and pre- and post-conditions, placing 
a high annotation burden on the programmer.
%
The second class of approaches design \emph{abstract interpretations} 
tailored to particular data
structures~\cite{TVLA,cookCAV08,changPOPL08,BerdineCAV11}, 
to enable the automatic inference of invariants, but they cannot be 
\emph{extended by users}, to new kinds of structures and properties.

In this paper, we reconcile extensibility and inference 
using \emph{Alias Refinement Types} (\toolname). 
%
The key insight in \toolname, is that we can 
\emph{factor} the specification and verification 
of data structure invariants into two orthogonal 
components: 
%
a \emph{physical} component describing the basic 
shape and linkages of the \emph{structures} and
%
a \emph{logical} component describing semantic 
or relational properties of the \emph{data} contained 
within them.

Thus, our first contribution is to use the above insight 
to develop \toolname~(\S~\ref{sec:check}) by carefully 
composing two well known, but orthogonal techniques.
%
To represent the physical structure of the 
heap we use \emph{alias types}\cite{AliasTypesRec}, 
which augment a standard type checker with locations, 
and a mutable heap that maps locations to records 
or collections, thereby precisely tracking the shape
of the heap in the presence of aliasing and mutation.
%
To represent the logical properties and relationships
of heap structures, we introduce heap binders
that name the contents of locations, and then 
decorate types with \emph{refinement predicates}
from SMT decidable theories \cite{Rushby98,XiPfenning99}.

Our second contribution is to show how \toolname enables 
inference(\S~\ref{sec:infer}) by partitioning the work into 
%
(a)~the physical alias type system that can reconstruct the 
    shape of the heap at each program point from the simple, 
    unrefined, function type specifications, and,
%
(b)~the refinement type system that uses the technique of 
    liquid typing\cite{LiquidPLDI08} to synthesize the 
    decorating refinements from a user-supplied set of 
    logical qualifiers, thereby inferring correctness invariants.

Our third contribution is a novel soundness proof technique.
%
We connect the type system of \toolname to separation logic
proofs~\cite{???}:
%
By providing an interpretation of the type system in separation logic,
we show that the type judgements correspond to implications in
separation logic.
%
Central to our interpretation is the insight that heap binders
correspond to pure (\ie heap-independent) \emph{snapshots} of
the heap.
%
Thus, invariants that describe logical properties and relationships
between heap structures actually correspond to relationships between
different snapshots of the heap.

Our fourth contribution is an implementation and evaluation
of \toolname~(\S~\ref{sec:eval}).
%
We describe how \toolname allows us to define a variety 
of linked data structures, including singly linked lists, 
doubly linked lists, cyclic lists, heaps and red-black trees.
%
Finally, we show how we can use type refinements to specify 
and verify a variety of functional correctness properties 
of linked structures. The properties range from the 
sizes and sets of elements of lists, to a variety of 
list-sorting algorithms, to height balanced-ness, heap- and 
binary-search ordering and red-black coloring invariants, 
demonstrating the extensibility and automation of 
our approach.

\rj{INTRO}
We formally prove that \toolname is a stylized instance of separation logic,
and show that each the heap-binders to which we crucially associate functional 
correctness properties (via measures) correspond to pure snapshots 
(\ie \emph{auxiliary} or \emph{ghost}) values in the program logic.
Furthermore, the alias type system allows us to update the heap 
\emph{locally} at pointer writes, \emph{folds} or \emph{unfolds}.
This eliminates the problem of having to reason about transitive 
reachability, and hence lets \toolname overcome the primary obstacle
towards automating the verification of linked data structures.

\rj{INTRO}
Note that we use this translation \emph{only} to prove soundness, 
and \emph{not} in our actual verification algorithm.
That is, rather than use the usual preservation-and-progress route,
we show that our type system can be viewed as a stylized subset of
separation logic with the benefit of having:
%
\begin{inparaenum}[(1)]
\item easy programmer extensibility through type definitions, and
\item automatic property checking and inference 
\end{inparaenum}
%
without requiring specialized recursive separation logic predicates,
axioms, decision procedures, or abstract transformers, all of which 
we get for free, via alias typing. 


\rj{INTRO}
\toolname's decoupling of the heap from refinements makes 
it possible to use off-the-shelf SMT solvers to infer refinements.
%
As the qualifiers are simple (non-separation logic) predicates, 
they may, in future work, be automatically computed via CEGAR \cite{hmc}.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> lang.tex <==
\section{Language}\label{sec:lang}

We begin by presenting a standard imperative language, \lang,
with records and the usual call-by-value semantics.

\subsection{Syntax}
\begin{figure}[t!]
\input{syntax} 
\input{types2}
\caption{Syntax of \lang programs and types}
\label{fig:syntax}
\label{fig:types}
\end{figure}

\Cref{fig:syntax} summarizes the syntax of \lang programs.
A program in \lang is a sequence of functions, each comprising 
statements composed of expressions.

\mypara{Expressions}
The pure expressions of \lang are do not depend on
heap-stored values. These include integer and boolean constants, variables
and pure operations on the above (\eg addition, subtraction, comparison, \etc.)
We include references which only appear inside the elaborated fold and
unfold annotations.

\mypara{Statements}
The statements of \lang include all the possible constructs that may 
manipulate the heap. These include the usual assignment, record allocation, 
field read and write, conditionals, function calls and returns, all of which
can be composed via sequencing. (For simplicity, \lang eschews loops in favor
of recursion.)

\mypara{Annotations} 
In \lang, reasoning about heap-allocated data structures is made possible
by the \emph{ghost} statements \windName, \unwindName, \concName, and \padName.
%
These annotations \emph{do not appear} in the source program -- instead 
\toolname automatically inserts these in an elaboration phase, prior to
refinement type inference \S~\ref{sec:infer}. 
%
The annotations have no effect on the \emph{dynamic} semantics of a 
\lang program. Instead, they serve as anchors for \emph{statically} 
tracking the shape of the program's heap.

\subsection{Types}

% \input{types2}

\Cref{fig:types} summarizes the syntax of \lang types, 
which include unrefined types \tbase, refinement types \ty, 
heaps \heap, and functions \funschema.

\mypara{Types}
The types of \lang include integers, booleans, type variables 
and (possibly null) references. In addition, \lang supports 
record types \ie sequences of field-type pairs, and instances
of user-defined types which introduce a way to create linked
collections of heap-allocated structures.

\mypara{Refinement Types}
Values in \lang are given \emph{refinement types} 
\cite{Rushby98,XiPfenning99}, which join an (unrefined) type 
\tbase with a logical predicate \pred drawn from a decidable
theory. The the \emph{value variable} \vv refers to the value
of the expression being typed, and so \reft describes
all \vv of type \tbase that satisfy \pred \cite{Knowles10}.

\mypara{References} 
%
In \lang, \emph{locations}, \loc, denote heap addresses.
%
Each location \loc is an abstraction of a \emph{single} 
run-time heap address (and not a \emph{summary} of multiple 
addresses).
%
A location \loc may be read and written via 
a reference with type $\tref{\loc}$.

\mypara{Heaps} 
%
A \emph{heap} is an \emph{unordered} collection of mappings from
locations, \loc, to bound types (\vartybind).
%
In \lang, A heap \heap is described by a set of \emph{bindings} of the
form \hplocty{\loc}{\evar}{\ty} joined using the \hpjoin operator.
%
The binding \hplocty{\loc}{\evar}{\ty} denotes a heap that maps the
location \loc to the type \ty bound to the variable \evar.
%
This type, \ty, describes the possible values that appear at
the memory address denoted by \loc.
%
The name $\evar$ may appear in refinement formulas in order to express
dependency on values stored at \loc.
%
We let $\dom{\heap}$ denote the set of locations mapped in \heap.

\mypara{Type Definitions}
%
To define heap-allocated data structures, \lang allows 
recursive type definitions.
%
A definition
     \tydef{\tyapp{\tycon}{\many{\tvar}}}
                         {\heap}
                         {\evar}
                         {\tobj{\many{\field:\ty}}}
 consists of four components:
\begin{inparaenum}[(1\upshape)]
  \item a name, \tycon;
  \item $\many{\tvar}$, a sequence of type variables that paramaterize the the type;
  \item $\heap$, an existentially quantified heap; and
  \item $\tybind{\evar}{\tgenobj{\field}{\ty}}$, a record.
\end{inparaenum}

\mypara{Function Schemas}
%
A \emph{schema}
$
\quant{\many{\loc,\tvar}}
 \funty{\many{\tybind{\evar}{\ty}}}{\heap}{\equant{\many{\loc'}}\tybind{\evar'}{\ty'}}{\heap'}
$
describes a function that takes arguments $\many{\evar}$ in a
heap satisfying $\heap$ and returns a value of type $\ty'$.
%
Side effects are captured by the \emph{output} heap, $\heap'$.
%
Functions are parameterized by type variables, $\many\tvar$, and
locations $\many\loc$.
%
Locations allocated by the function are
\emph{existentially} quantified (the $!$ states the locations are distinct
from existing heap locations).
%
The schema
$
\funty{\tybind{x}{\tint}}{\hpemp}{\equant{\loc}\tb{y}{\tref{\loc}}}
      {\hplocty{\loc}{z}{\tobj{\tybind{n}{\reftp{\tint}{\vv = x}}}}}
$
denotes a function that returns a pointer to a new record containing an 
\tint field equal to the function's argument.

%%% Local Variables: 
%%% mode: latex
%%% eval: (TeX-PDF-mode 1)
%%% TeX-master: "main.tex"
%%% End: 


==> oldcommands.tex <==
\newcommand{\techrep}[1]{}

%\def\mynote#1{{\sf $\clubsuit$ #1 $\clubsuit$}}
%\def\mynote#1{{}}
%\newcommand{\mynote}[2]{{\sf {#1} $\clubsuit$ {#2} $\clubsuit$}}
\newcommand{\mynote}[2]{}
\newcommand{\pmr}[1]{\mynote{pmr}{#1}}
\newcommand{\mk}[1]{\mynote{mk}{#1}}
\newcommand{\rj}[1]{\mynote{rj}{#1}}
\newcommand{\abakst}[1]{\mynote{abakst}{#1}}

\newcommand{\regleq}{\sqsubseteq}
\newcommand{\regeq}{\equiv}
\newcommand{\regfiner}{\unlhd}

\newcommand{\st}{\; | \;}
\newcommand{\fa}{\forall \,}
\newcommand{\ex}{\exists \ }
\newcommand{\defeq}{\stackrel{\cdot}{=}}
\newcommand{\bottom}{\perp}
\newcommand{\dbrkts}[1]{[\![#1]\!]}
\newcommand{\refine}[1]{\Delta}
\newcommand{\ie}{{\it i.e.,~}}
\newcommand{\eg}{{\it e.g.~}}
\def\etc{{\it etc.}}

\newcommand{\pair}[2]{{({#1}, {#2})}}

\newcommand{\prog}{\mathit{P}}
\newcommand{\err}{\mathcal{E}}
\newcommand{\init}{\mathcal{I}}
\newcommand{\safe}{\mathcal{S}}
\def\T{{\mathcal{T}}} %check
\def\G{{\mathcal{G}}} %check


\def\tar{{\sc Tar~}}
\def\hytech{{\sc HyTech}}
\newcommand\blast{{\sc Blast}\xspace}
\newcommand\tblast{{\sc Blast-Test}\xspace}
\newcommand{\nesc}{{\sc nesC}\xspace}

\def\etar{{\sf CIRC}}
\def\lazyabs{\mathsf{LazyAbstraction}}
\def\symbrr{\mathsf{SymbReachRefine}}

\def\pred{\varphi}

\def\true
\def\false{{\it false}}

\newcommand{\lts}{\mathcal{S}}

\newcommand{\states}{S}
\newcommand{\state}{s}
\newcommand{\astate}{t}
\newcommand{\absstate}{\hat{s}}
\newcommand{\ob}{\pi}
\newcommand{\obs}{\Pi}
\newcommand{\STATES}{{\it States}}
\newcommand{\FORMULAS}{\it FOL}

\newcommand{\TERMS}{\it TERMS}
\newcommand{\ATP}{\it ATOMS}




\def\mem{{\it Mem}}
\def\Reg{{\mathit{R}}}
%\def\val{{\mathit{v}}}
\def\val{\mathsf{V}}
\newcommand{\FOL}{{\it FOL}}

\newcommand{\ExpSet}{\mathsf{Exp}}
\newcommand{\PredSet}{\mathsf{Pred}}
\newcommand{\OpSet}{\mathsf{Op}}
\newcommand{\LVALS}{\mathsf{Lvals}}
\newcommand{\TypeSet}{\mathsf{Typ}}
\newcommand{\OPERATIONS}{\OpSet}


\newcommand{\CMDS}{\mathit{Cmd}}
\newcommand{\TYPES}{\mathsf{Types}} 
\newcommand{\EXPRS}{\ExpSet} 
\newcommand{\BEXPRS}{\PredSet}
\newcommand{\DECLS}{{\it Decl}} %check
\newcommand{\PRGM}{{\it Prgm}} %check
\newcommand{\TRACES}{{\it Traces}} %check
\newcommand{\constr}{\it constraints} %check



\newcommand{\CFA}{\mathit{C}}


\newcommand{\ACFA}{\mathit{A}}


\def\op{{\mathsf{op}}}
\def\pop{{\mathsf{pop}}}
\newcommand{\oper}{\mathtt{o}}

\newcommand{\PC}{{\it PC}}




\newcommand{\atomic}{\mathit{Atomic}}
\newcommand{\atp}{\mathit{At}}
\newcommand{\atloc}{\mathit{AL}}
\newcommand{\loc}{\mathit{L}}
\newcommand{\Qat}{Q^*}

\newcommand{\ttzero}{\mathtt{0}}
\newcommand{\ttx}{\mathtt{x}}
\newcommand{\tty}{\mathtt{y}}
\newcommand{\ttY}{\mathtt{Y}}
\def\tte{\mathtt{e}}
\def\ttp{\mathtt{p}}
\def\ttl{\mathtt{l}}
\def\ttasg{\mathtt{:=}}

\newcommand{\REF}{{\tt ref\ }}
\newcommand{\typ}{{\sf{typ}}}
\newcommand{\sel}{{\tt sel}}
\newcommand{\upd}{{\tt upd}}
\newcommand{\type}{{\it type}}
\newcommand{\CHLVAL}{{\it ChLval}}
\newcommand{\chlval}{{\it cl}}

\newcommand{\sym}{{\it sym}}
\def\Cl{{\it Cl}}

\newcommand{\ls}{\mathit{ls}} %check
\newcommand{\enabled}[1]{\mathit{enabled}_{#1}} %check
\newcommand{\con}[1]{\overline{#1}} %check



\def\learn{{\sf Extract}}
\def\focus{\Phi}
%\def\learn{{\sf Extract}}
\def\learn{\focus}
\def\pone{{\sf PI}}
\def\ptwo{{\sf PII}}
\def\pthree{{\sf PIII}}
\def\pfour{{\sf PIV}}

%code

\def\pc{{\it pc}}
\def\stk{{\it cs}}
\newcommand{\pcs}{\mathit{pcs}}
\def\ASSUME{{\mathtt{assume}}~}
\def\assume{\ASSUME~}

\def\RETURN{{\mathtt{return}}}
\def\SKIP{{\mathtt{skip}}}
\def\If{{\mathtt{if}}}
\def\main{{\mathtt{main}}}	
\def\int{{\mathit{Int}}}	
\def\addr{{\it Addr}}
\def\reference{{\mathtt{ref}}}	
 
\def\fun{f}

\def\foo#1{}
\newcommand{\svars}{\mathit{Shared}}
\newcommand{\pvars}[1]{\mathit{Private}_{#1}}

\newcommand{\reads}[2]{\mathit{Read}_{#2}({#1})}
\newcommand{\extend}[2]{{\cal E}_{#1}(#2)}

\newcommand{\TRANS}{{\rightarrow}}
\def\trans{{\delta}}
\newcommand{\Pre}{\mathsf{Pre_{\lts}}}
\newcommand{\Post}{\mathsf{Post_{\lts}}}
\newcommand{\pre}{\mathsf{pre}}
\newcommand{\post}{\mathsf{post}}
\newcommand{\abspre}{\widehat{\pre}}
\newcommand{\abspost}{\widehat{\post}}
\newcommand{\PImage}{\widehat{\post}}
\newcommand{\reach}{{\sf Reach}}
\newcommand{\ena}{{\sf En}}
\def\WP{\mathsf{WP}}
\def\SP{\mathsf{SP}}
\def\SPD{\mathsf{SP^D}}
\def\ABSSPD{\widehat{\SPD}}

\def\goesto#1{\smash{\stackrel{#1}{\leadsto}}}
\def\labarrow#1{\smash{\xrightarrow{#1}}}


\def\SPF#1{\mathsf{SP}_{#1}}
\def\SPC{\SPF{\Pi}}
\def\SPP{\SPF{P}}
\def\abs{\mathsf{\alpha}}


\def\set#1{{\{ #1 \}}}
\def\zug#1{{\langle #1 \rangle}}
\newcommand{\transrel}{\leadsto}

\newcommand{\gloeq}{\approx}
\newcommand{\gloleq}{\lesssim}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% Primitive functions used in the algorithm \learn %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\UPDATEMAP{{\sf{Upd}}}
\def\CONS{{\sf{Con}}}
\def\INTERPOLANT{{\sf{Interpolant}}}
\def\clean{{\sf{Clean}}}
\def\Atoms{{\sf{Atoms}}}
\def\context{{\sf{Context}}}
\newcommand{\SUBS}{{\sf{Sub}}}
\newcommand{\refclose}{{\sf{clos^*}}}
\newcommand{\equate}{{\sf{Equate}}}
\newcommand{\eqaddr}{{\sf{EqAddr}}}
\newcommand{\alias}{{\sf{Alias}}}
\newcommand{\aliases}{{\sf{Aliases}}}
\newcommand{\ASGN}{{\sf{Asgn}}}
\newcommand{\new}{{\sf New}}
\newcommand{\ite}{{\sf{ite}}}
\newcommand{\Copy}{{\sf{copy}}}
\newcommand{\diff}{{\sf{diff}}}


%\newcommand{\Itp}[3]{\mbox{\sc Itp}^{(#2,#3)}(#1)}
\newcommand{\SeqItp}[4]{(#1,#2) \vdash #3 \ [#4]}
\newcommand{\SeqItpA}[4]{\vdash #3 \ [#4]}
\newcommand{\Soln}[2]{\mbox{\sc Soln}(#1,#2)}
\newcommand{\Cond}[2]{\mbox{\sc Cond}(#1,#2)}
\newcommand{\Rest}[2]{\mbox{\sc Rest}(#1,#2)}
\newcommand{\Itp}[3]{\smash{\mbox{\sc Itp}{.(#2,#3).}}(#1)}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% Primitive functions used in the algorithm \etar %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\check{{\mathsf{Check}}}
%% ConcurrentReachabilityAbstractionCheck with K 
\def\collapse{{\mathsf{Collapse}}}
\def\reach{{\mathsf{Reach}}}
\def\issafe{{\mathsf{Safe}}}
\def\reachandbuild{{\mathsf{ReachAndBuild}}}
\def\modelcheck{{\mathsf{ModelCheck}}}
\def\checksim{{\mathsf{CheckSim}}}
\def\refine{{\mathsf{Refine}}}
\def\exc{{\mathsf{Exception}}}
\def\findpath{{\mathsf{FindPath}}}
\def\connect{{\mathsf{Connect}}}
\def\addedge{{\mathsf{AddEdge}}}
\def\union{{\mathsf{Union}}}
\def\find{{\mathsf{Find}}}

\def\abs{{\mathsf{Abs}}}
\def\adr{{\mathsf{AbsDataReg}}}
\def\safe{{\sc{Safe}}}
\def\unsafe{{\sc{Unsafe}}}
\def\real{{\text{\sc Real~}}}


%%%%% Also used in ETAR -- variables ?
\def\acc{{\mathcal{A}}} %check

%% macros for examples
\newcommand{\lockb}{{\it LOCK}}
\newcommand{\locks}{{\it lock}}
\newcommand{\locktt}{\mathtt{lock()}}
\newcommand{\unlocktt}{\mathtt{unlock()}}
\newcommand{\newb}{{\it new}}
\newcommand{\oldb}{{\it old}}
\newcommand{\ret}{{\it ret}}
\def\flag{\mathit{flag}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%    Notation for Trees/Graphs etc  %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\node{\mathtt{n}}
\newcommand{\leaf}{\mathit{Leaf}}
\newcommand{\intl}{\mathit{Intl}}
\def\tree{T}


\newcommand{\valid}{\vdash}
\newcommand{\vc}{\mathsf{VC}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%    MACROS for PROOFS etc.  %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\renewcommand{\implies}{\Rightarrow}
\renewcommand{\iff}{\Leftrightarrow}
% Proof rules
\def\pf{\mathtt{pf}}
\def\falsee{\mathtt{falsee}}
\def\andi{\mathtt{andi}}
\def\ande{\mathtt{ande}}
\def\alli{\mathtt{alli}}
\def\impdist{{\text{\tt imp-dist}}}
\def\ori{\mathtt{ori}}
\def\oril{\mathtt{oril}}
\def\orir{\mathtt{orir}}
\def\ore{\mathtt{ore}}
\def\impi{\mathtt{impi}}
\def\impe{\mathtt{impe}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% THESE SHOULD GO 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\vars{V}
\newcommand{\rjreach}{Reach} %%%%% THIS ONE SHOULD GO!
%\def\smallfont#1{\begin{small} #1 \end{small}}
\def\smallfont#1{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Random defs needed by tests_from_counterexamples %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tpred}{p}
\newcommand{\tq}{q}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% Bit Vector Types %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\lshift{{<\!<}}
\def\rshift{{>\!>}}
\def\bvt{T}
\def\solve{\mathsf{Solve}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% Unclassified %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\prediset{\Lambda}
\def\predmap{\Pi}
\def\param{\mathit{par}}
\def\valu{\nu}
\def\store{m}
\def\mem{M}
\def\trace{\sigma}
\def\funs{F}
\def\assm#1{\mathtt{assume [#1]}}
\def\cmd{l}


\def\seen{Seen}
\def\keeptree{\mathsf{KeepSubtree}}
\def\mybad{bad~}
\def\ctr{{\it ctr}}
\def\inc{{\tt inc}}
\def\tf{\mathsf{TF}}
\def\scolon{\!:\!}
\def\dblcolon{\!::\!}
\def\mreach{\mathsf{Mreach}}
\def\initc{\mathsf{IC}}

\def\myjoin{\otimes}
\def\mprog{\overline{\prog}}
\def\mlts{\overline{\lts}}
\def\thread{\lts}
\newcommand{\simu}{\preceq}
\def\asimu{\simu}
\def\issafe{\mathsf{Safe}}
\def\pool{\mathsf{Pool}}
\def\context#1{{#1}^{\omega}}
\newcommand{\locals}[1]{{#1}_L}
\newcommand{\globals}[1]{{#1}_G}
\def\tcp#1#2{\mathsf{TCP}.(#1,#2)}
\def\symabs#1{\mathcal{A}_{#1}} % do not change
\def\symreg#1{\mathcal{R}_{#1}}
\def\havoc{\mathsf{Havoc}}
\def\havabs#1{\mathcal{H}_{#1}}
\def\abshavoc{\widehat{\havoc}}
\def\AT{A}
\newcommand{\writes}[2]{\mathsf{Write}_{#1}({#2})}
\newcommand{\contabs}[2]{\mathsf{ContAbs}.{#1}.{#2}}
\def\ctrmaps{\Delta}
\def\ctrmap{\delta}
\def\tcpabs#1#2#3{\mathsf{TCPabs}.(\thread,\symreg{\thread}).(\AT,k)}

\def\tcr{R^{\omega}}
\def\tcdbrkts#1{\dbrkts{#1}^{\omega}}
\def\tcpost{\abspost^{\omega}}
\def\thread{T}
%\def\proj{\downarrow}
\def\wrt{\mathsf{Write}}
\def\myzap#1{}
\def\fmain{\fun_{\mathtt{main}}}



\newcommand{\cfa}{{\mathsf{cfa}}}
\newcommand{\mgc}{{\mathsf{mxc}}} % most general client
\def\interface{{\mathsf{IntfP}}}
\def\flt{{\mathsf{Flat}}}
\newcommand{\property}{{\mathsf{Prop}}}

\def\Reg{\mathcal{R}}
\def\dom{\mathit{Dom}}
\def\acc{{\mathcal{A}}}
\def\accNodes{\mathrm{accNodes}}
\def\nodeSet{\mathrm{NodeSet}}
\def\flag{\mathit{flag}}

\def\obsf#1{\langle\!\langle #1 \rangle\!\rangle}
\def\ext#1{\ulcorner #1 \urcorner}

\def\T{{\mathcal{T}}}
\def\G{{\mathcal{G}}}

% the real pre and post
\def\buildinterface{{\mathsf{BuildInterface}}}
\def\fold{{\mathsf{fold}}}
\def\witness{{\mathsf{witness}}}
\def\reals{\mathbb{R}}
\def\nats{\mathbb{N}}
\def\ints{\mathbb{Z}}

\def\concat{{.}}
\def\translate{{\mathsf{translate}}}
\def\aname{{\mathsf{a}}}
\def\bname{{\mathsf{b}}}
\def\cname{{\mathsf{c}}}
\def\dname{{\mathsf{d}}}
\def\ename{\mathsf{e}}
\def\fname{\mathsf{f}}
\def\gname{\mathsf{g}}
\def\hname{\mathsf{h}}
\def\kname{\mathsf{k}}
\def\mname{\mathsf{m}}
\def\nname{\mathsf{n}}
\def\oname{\mathsf{o}}
\def\pname{\mathsf{p}}
\def\qname{\mathsf{q}}
\def\rname{\mathsf{r}}
\def\sname{\mathsf{s}}
\def\tname{\mathsf{t}}
\def\uname{\mathsf{u}}
\def\vname{\mathsf{v}}
\def\wname{\mathsf{w}}
\def\op{\oplus}
\def\bop{\wedge}
\newcommand{\arrin}[1]{#1\_{\mathsf{idx}}}
\newcommand{\arrout}[1]{#1\_{\mathsf{elem}}}
\def\names{\mathbb{A}}
\def\blocks{\mathbb{B}}
\newcommand{\blk}[2]{\zug{#1,#2}}
\def\size{\ell}
\def\block{b}
\def\bvt{\bar{b}}
%\newcommand{\proj}[2]{#1 \downarrow #2}

\newcommand{\bound}[2]{{\mathsf{Bound}(#1,#2)}}
\newcommand{\proj}[2]{#1[#2]}
\newcommand{\bproj}[2]{#1 #2}
\def\tv{\tau}
\def\tvs{{\mathbb{T}}}
\newcommand{\itv}[2]{[#1:#2]}
\def\tasgn{T}
\newcommand{\udef}[3]{(#1,#2,#3)}
\def\bvle{\leq}
\def\expn{\sigma}
\def\zname{\mathbf{0}}
%\def\zb{\blk{\zname}{1}}
\def\zb{\zname}
\def\unify{{\mathsf{Unify}}}
\def\subalign{{\mathsf{Subalign}}}
\def\split{{\mathsf{Split}}}
\def\zsol{{\mathsf{T_0}}}
\def\single{{\mathsf{Single}}}
\def\con{{\mathsf{Con}}}
\def\barrow{{\mathbf{\longrightarrow}}}
\def\gnode{v}
\def\sequence{{\mathsf{Seq}}}
\def\find{{\mathsf{Find}}}
\def\tvp{\tv_{\mathtt{p}}}
\def\tvpone{\tv_{\mathtt{p \& 1}}}
\def\tvptwenty{\tv_{\mathtt{p \& 1^{20}0^{12}}}}
\def\tvpten{\tv_{\mathtt{p \& 1^{10}0^2}}}
\def\tvptwelve{\tv_{\mathtt{p1 \rshift 12}}}
\def\tvpten{\tv_{\mathtt{p \& 1^{10}0^2}}}
\def\tvpo{\tv_{\mathtt{p1}}}
\def\tvpte{\tv_{\mathtt{pte}}}
\def\tvbo{\tv_{\mathtt{b1}}}
\def\tvbothirty{\tv_{\mathtt{b1 \& 1^{30}0^2}}}
\def\tvbase{\tv_{\mathtt{base}}}
\def\tvoff{\tv_{\mathtt{off}}}
\def\tvbasoff{\tv_{\mathtt{base+off}}}
\def\tva{\tv_{\mathtt{a}}}
%\def\tvmin{\tv_{\mathtt{m\_idx}}}
%\def\tvmout{\tv_{\mathtt{m\_elem}}}
%\def\tvtabi{\tv_{\mathtt{tab\_idx}}}
%\def\tvtabo{\tv_{\mathtt{tab\_elem}}}
\def\tvmin{\tv_{\arrin{\mathtt{m}}}}
\def\tvmout{\tv_{\arrout{\mathtt{m}}}}
\def\tvtabi{\tv_{\arrin{\mathtt{tab}}}}
\def\tvtabo{\tv_{\arrout{\mathtt{tab}}}}



\def\tvret{\tv_{\mathtt{mget\_r}}}

\def\ift{\mathtt{if}}
\def\thent{\mathtt{then}}
\def\elset{\mathtt{else}}
\def\while{\mathtt{while}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Macros added by Sorin %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\LVal}{\mathit{LVal}}
\newcommand{\Node}{\mathit{Node}}
\newcommand{\PPoint}{\mathit{PPoint}}
\newcommand{\FactName}{\mathit{FactName}}
\newcommand{\DataflowFacts}{\mathit{DataflowFact}}
\newcommand{\fact}{\mathit{f}}
\newcommand{\lval}{\mathit{lval}}
\newcommand{\shortlval}{\mathit{l}}
\newcommand{\SeqFlowFunc}{\mathit{F}}
\newcommand{\Domain}{\mathit{D}}
\newcommand{\Adjust}{\mathit{Adj}}
\newcommand{\AdjustedFlowFunc}{\mathit{F_{Adj}}}
\newcommand{\n}{\mathit{n}}
\newcommand{\dataflowinfo}{\mathit{d}}
\newcommand{\outpp}{\mathit{out\_pp}}
\newcommand{\pp}{\mathit{p}}
\newcommand{\rreg}{\mathit{r}}
\newcommand{\RacyRead}{\mathit{RacyRead}}
\newcommand{\Bool}{\mathit{Bool}}
\newcommand{\RaceRegion}{\mathit{Reg}}
\newcommand{\R}{\mathit{R}}
\newcommand{\arity}{\mathit{arity}}
\newcommand{\IPRegion}{\mathit{IPReg}}
\newcommand{\Regions}{\mathit{Regs}}
\newcommand{\Regionsplus}{\Regions_+}
\newcommand{\Regionsminus}{\Regions_-}
\newcommand{\Relay}{\textsc{Relay}\xspace}
\newcommand{\lvals}{\mathit{lvals}}
\newcommand{\proc}{\mathit{g}}
\newcommand{\SetOfAllLocks}{\mathit{L}}
\newcommand{\Pred}{\mathit{Pred}}
\newcommand{\ttg}{\mathtt{g}}
\newcommand{\ttfoo}{\mathtt{foo}}
\def\lplus{L_{+}}
\def\lminus{L_{-}}
\newcommand{\setv}[1]{\mathbb{#1}}
\newcommand{\RealRace}{\mathit{RealRace}}
\newcommand{\SumReg}{\mathit{SumReg}}
\newcommand{\IPRacyRead}{\mathit{IPRacyRead}}
\newcommand{\CallSite}{\mathit{CS}}
\newcommand{\cs}{\mathit{cs}}
\newcommand{\RacyKill}{\mathit{ThreadKill}}
\newcommand{\MustPointTo}{\mathit{MustPointTo}}
\newcommand{\HasConstantValue}{\mathit{HasConstantValue}}
\newcommand{\ttGzero}{\mathtt{G0}}
\newcommand{\ttGone}{\mathtt{G1}}
\newcommand{\region}{\mathit{r}}
\newcommand{\RelayResults}{\mathit{RelayResults}}
\newcommand{\dontcare}{\_}

\newcounter{indentenumcount}
\newenvironment{indentenum}{\begin{list}
   {\arabic{indentenumcount}.}
   {\usecounter{indentenumcount}
    \setlength{\parsep}{0pt}
    \setlength{\leftmargin}{30pt}
   } 
  }
  {\end{list}}

\newcommand{\Fun}{\setv{F}}
\newcommand{\Rename}{\mathit{Rename}}
\newcommand{\LockUpdate}{\mathit{LockUpdate}}
\newcommand{\Before}{\mathit{Before}}
\newcommand{\AllUnlocks}{\mathit{AllUnlocks}}
\newcommand{\trueout}{\mathit{true\_out}}
\newcommand{\RadarRelay}{$\algoname(\Relay)$\xspace}
%\newcommand{\RadarRelay}{\textsc{Radaray}\xspace}
\newcommand{\RadarRelayNoLocks}{$\algoname(\Relay_{\neg L})$\xspace}
\newcommand{\RadarSteens}{$\algoname(\textsc{Steens})$\xspace}
\newcommand{\Seq}{\textsc{Seq}\xspace}
\newcommand{\NNname}{\mathit{NonNull}}
\newcommand{\ApacheLineCount}{130,000\xspace}
\newcommand{\SSLLineCount}{210,000\xspace}
\newcommand{\LinuxLineCount}{830,000\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% RJ adding macros %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\ttf}{\ttname{f}}

\newcommand{\algoname}{\textsc{Radar}\xspace}
\newcommand{\ttprod}{\mathtt{Producer}}
\newcommand{\ttcons}{\mathtt{Consumer}}
\newcommand{\ttproduce}{\mathtt{produce}}
\newcommand{\ttperfc}{\mathtt{perf\_ctr}}
\newcommand{\ttbufs}{\mathtt{bufs}}
\newcommand{\ttpx}{\mathtt{px}}
\newcommand{\ttcx}{\mathtt{cx}}
\newcommand{\ttt}{\mathtt{t}}
\newcommand{\ttarr}{\mathtt{\rightarrow}}
\newcommand{\ttlock}{\mathtt{lock}}
\newcommand{\ttdata}{\mathtt{data}}
\newcommand{\ttflag}{\mathtt{flag}}

\newcommand{\ttbuflock}{\mathtt{buf\_lock}}
%\newcommand{\ttpxlock}{\mathtt{\ttpx \ttarr \ttlock}}
\newcommand{\ttpxdata}{\mathtt{\ttpx \ttarr \ttdata}}
\newcommand{\ttpxdatastar}{\mathtt{*\ttpxdata}}
\newcommand{\ttpxflag}{\mathtt{\ttpx \ttarr \ttflag}}
\newcommand{\ttcxflag}{\mathtt{\ttcx \ttarr \ttflag}}
%\newcommand{\ttcxlock}{\mathtt{\ttcx \ttlock}}
\newcommand{\ttcxdata}{\mathtt{\ttcx \ttarr \ttdata}}
\newcommand{\ttone}{\mathtt{1}}

\newcommand{\ttnew}{\mathtt{new}}


\newcommand{\ttPzero}{\mathtt{P0}}
\newcommand{\ttPone}{\mathtt{P1}}
\newcommand{\ttPtwo}{\mathtt{P2}}
\newcommand{\ttPthree}{\mathtt{P3}}
\newcommand{\ttPfour}{\mathtt{P4}}
\newcommand{\ttPfive}{\mathtt{P5}}
\newcommand{\ttPsix}{\mathtt{P6}}
\newcommand{\ttPseven}{\mathtt{P7}}
\newcommand{\ttPeight}{\mathtt{P8}}
\newcommand{\ttPnine}{\mathtt{P9}}
\newcommand{\ttPA}{\mathtt{PA}}
\newcommand{\ttCzero}{\mathtt{C0}}
\newcommand{\ttCone}{\mathtt{C1}}
\newcommand{\ttCtwo}{\mathtt{C2}}
\newcommand{\ttCthree}{\mathtt{C3}}
\newcommand{\ttCfour}{\mathtt{C4}}
\newcommand{\ttCfive}{\mathtt{C5}}
\newcommand{\ttCsix}{\mathtt{C6}}
\newcommand{\ttCseven}{\mathtt{C7}}
\newcommand{\ttCeight}{\mathtt{C8}}


\newcommand{\normsum}[1]{\normsumname({#1})}
\newcommand{\normsumname}{\mathit{Norm}}
\newcommand{\unmod}[1]{\mathit{NotMod}({#1})}
\newcommand{\NN}[1]{\mathit{NonNull}({#1})}
\newcommand{\ttnull}{\mathtt{NULL}}
\newcommand{\domelt}{d}
\newcommand{\Aliased}[2]{\mathit{Aliased}(#1,#2)}
\newcommand{\ttmalloc}{\mathtt{malloc(\ldots)}}

\newcommand{\parastart}[1]{\sk\noindent\emph{\textbf{#1 }}}

\newenvironment{sitemize}{\begin{list}
   {$\bullet$}
   {\setlength{\topsep}{2pt}
    \setlength{\itemsep}{2pt}
    \setlength{\leftmargin}{10pt}
    }

  }
  {\end{list}}

\newcommand{\sparagraph}[1]{\smallskip\noindent\emph{\textbf{#1}.}}
%% Para Formatting
\def\mypara#1{\sparagraph{#1}}
\newcommand{\program}[1]{\texttt{#1}}
\newcommand{\blankrow}[1]{\multicolumn{#1}{c}{}}
\newcommand{\kw}[1]{\textbf{#1}}
\newcommand{\seq}[1]{\overline{#1}}
\newcommand{\typbind}[2]{\ensuremath{{#1}: {#2}}}
\newcommand{\rulesheader}[2]{{\textbf{#1}} \hfill{\framebox{${#2}$}}}
\newcommand{\unsat}[1]{\ensuremath{\mathsf{Unsat}({#1})}}
\newcommand{\progvar}[1]{\ensuremath{\mathtt{#1}}}
\newcommand{\dunsat}[1]{\eff_{\mathsf{Unsafe}} = #1}
%%%%%% Liquid-Effects-Specific

\newcommand{\lang}{\ensuremath{LImp}\xspace}

%%%% Metavariables

%% Programs
\newcommand{\mvval}{\ensuremath{v}}
\newcommand{\mvaop}{\ensuremath{\circ}}
\newcommand{\mvrel}{\ensuremath{\sim}}
\newcommand{\mvpexpr}{\ensuremath{a}}
\newcommand{\mvexpr}{\ensuremath{e}}
\newcommand{\mvfundec}{\ensuremath{F}}
\newcommand{\mvprog}{\ensuremath{P}}

%% Indices
\newcommand{\mvindex}{\ensuremath{i}}
\newcommand{\mvindexseq}{\ensuremath{i^+}}

%% Locations
\newcommand{\mvlocname}{\ensuremath{l}}
\newcommand{\mvhloc}{\ensuremath{l}}
\newcommand{\absl}[1]{\ensuremath{\tilde{#1}}}
\newcommand{\concl}[2]{\ensuremath{{#1}_{#2}}}
\newcommand{\mvaloc}{\ensuremath{\absl{\mvhloc}}}
\newcommand{\mvcloc}[1]{\ensuremath{\concl{\mvhloc}{#1}}}

%% Heaps
\newcommand{\mvblock}{\ensuremath{c}}
\newcommand{\mvheap}{\ensuremath{h}}

%% Effects
\newcommand{\effempty}{\ensuremath{\epsilon}}
\newcommand{\mveffect}{\ensuremath{\Sigma}}
\newcommand{\mveffectset}{\ensuremath{\mathbb{E}}}
\newcommand{\mveffectname}{\ensuremath{E}}
\newcommand{\mvcommuteset}{\ensuremath{\mathbb{C}}}
\newcommand{\mveffectenv}[2]{\ensuremath{\pair{#1}{#2}}}

%% Refinement predicates
\newcommand{\mvrefpred}{\ensuremath{p}}

%% Types
\newcommand{\mveff}{\ensuremath{\Sigma}}
\newcommand{\mvtyp}{\ensuremath{b}}
\newcommand{\mvreftyp}{\ensuremath{\tau}}
\newcommand{\mvfunscm}{\ensuremath{\sigma}}
\newcommand{\mvfunscml}{\ensuremath{\tilde{\mvfunscm}}}


%%%% Expression forms

%% Values
\newcommand{\vptr}[1]{\ensuremath{\&{#1}}}
\newcommand{\vvoid}{\ensuremath{\mathtt{void}}}

%% Pure Expressions
\newcommand{\ptrplus}{\ensuremath{+_p}}

%% Effectful Expressions
\newcommand{\exlet}[3]{\ensuremath{\kw{let }{#1} = {#2} \kw{ in }{#3}}}
\newcommand{\exletu}[3]{\ensuremath{\kw{letu }{#1} = \kw{unfold }{#2} \kw{ in }{#3}}}
\newcommand{\exfold}[1]{\ensuremath{\kw{fold }{#1}}}
\newcommand{\exmalloc}[1]{\ensuremath{\kw{malloc} ({#1})}}
\newcommand{\exite}[3]{\ensuremath{\kw{if }{#1}\kw{ then }{#2}\kw{ else }{#3}}}
\newcommand{\exread}[1]{\ensuremath{*{#1}}}
\newcommand{\exwrite}[2]{\ensuremath{*{#1} := {#2}}}
\newcommand{\expar}[2]{\ensuremath{{#1}\parallel{#2}}}
\newcommand{\exforeach}[4]{\ensuremath{\kw{for each }{#1}{\kw { in }{#2}\kw{ to }{#3}\ \{{#4}\}}}}

%% Function Declarations
\newcommand{\fundec}[3]{{#1}\ ({#2})\ \{\ {#3}\ \}}

%%%% Types

%% Base types
\newcommand{\tyname}[1]{\mathtt{#1}}
\newcommand{\tyint}[1]{\ensuremath{\tyname{int}({#1})}}
\newcommand{\typtr}[2]{\ensuremath{\tyname{ref}({#1}, {#2})}}

%% Refined types
\newcommand{\reftyp}[2]{\ensuremath{\set{\valu:\ {#1}\ \mid\ {#2}}}}
\newcommand{\sreftyp}[1]{\set{{#1}}}
\newcommand{\unreftyp}[1]{{#1}^{\top}}



%% Predicates
\newcommand{\pfalse}{\ensuremath{\mathrm{false}}}
\newcommand{\ptrue}{\ensuremath{\mathrm{true}}}

%% Indices
\newcommand{\indexseq}[2]{\ensuremath{{#1}^{+{#2}}}}

%% Locations

%% Effects
\newcommand{\eempty}{\ensuremath{\varepsilon}} % pmr: collides with hempty
\newcommand{\eseq}{\ensuremath{\oplus}}
\newcommand{\ebind}[2]{\ensuremath{{#1} \mapsto {#2}}}
\newcommand{\ejoin}{\ensuremath{*}}
\newcommand{\eext}[3]{\ensuremath{{#1} \ejoin \ebind{#2}{#3}}}
\newcommand{\opeproject}{\ensuremath{\pi}}
\newcommand{\eproject}[2]{\ensuremath{\opeproject({#1}, {#2})}}
\newcommand{\opeinject}{\ensuremath{\mathit{logEffect}}}
\newcommand{\einject}[2]{\ensuremath{\opeinject({#1}, {#2})}}

%% Heaps
\newcommand{\indexbind}[2]{\ensuremath{{#1}: {#2}}}
\newcommand{\hempty}{\ensuremath{\varepsilon}}
\newcommand{\hjoin}{\ensuremath{*}}
\newcommand{\hbind}[2]{\ensuremath{{#1} \mapsto {#2}}}
\newcommand{\hext}[3]{\ensuremath{{#1} \hjoin \hbind{#2}{#3}}}

%% Worlds
\newcommand{\inheap}[2]{\ensuremath{{#1}/{#2}}}
\newcommand{\inworld}[2]{\ensuremath{\inheap{#1}{#2}}}

%% Function schemas
\newcommand{\funtyp}[4]{\ensuremath{\inheap{({#1})}{#2}\ \rightarrow\ \inworld{#3}{#4}}}
\newcommand{\funscm}[2]{\ensuremath{\forall {#1}.\ {#2}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Language Syntax
\newcommand{\ttcode}[1]{\ensuremath{\mathtt{#1}}}
\newcommand{\ttname}[1]{\ensuremath{\mathtt{#1}}\xspace}

\newcommand{\ttif}{\ttname{if}}
\newcommand{\ttthen}{\ttname{then}}
\newcommand{\ttelse}{\ttname{else}}

\newcommand{\ttchar}{\ttname{char}}
\newcommand{\ttint}{\ttname{int}}
\newcommand{\ttbool}{\ttname{bool}}
\newcommand{\ttshort}{\ttname{short}}
\newcommand{\ttvoid}{\ttname{void}}

\newcommand{\ttlet}{\ttname{let}}
\newcommand{\ttletf}{\ttname{letf}}
\newcommand{\ttletu}{\ttname{letu}}
%\newcommand{\ttletrec}{\ttname{let\ rec}}

%\newcommand{\aop}{+}
%\newcommand{\pop}{+_p}
%\newcommand{\prel}{\sim}
%
%\newcommand{\BIN}[3]{{#1}\ {#2}\ {#3}}
%
%\newcommand{\ttrestrict}{\ensuremath{\mathtt{restrict}}}
\newcommand{\ttassert}{\ttname{assert}}
%\newcommand{\ASSERT}[1]{\ttassert({#1})}
%\newcommand{\ttmalloc}{\ttname{malloc}\xspace}
%\newcommand{\ttnew}{\ttname{new}\xspace}
\newcommand{\MALLOC}[2]{\ttmalloc({#1},{#2})}
\newcommand{\NULL}[2]{\mathtt{NULL}_{{#1},{#2}}}

\newcommand{\UFAPP}[2]{{#1}({#2})}
\newcommand{\CALL}[3]{[#1]\ {#2}({#3})}
\newcommand{\RCALL}[3]{{#2}({#3})}

\newcommand{\ttin}[0]{\ttname{in}}
\newcommand{\ttfun}{\mathtt{fun}}
\newcommand{\FUN}[3]{\ttfun({#1})\{ {#2} \} : {#3}}
\newcommand{\ITE}[3]{{\ttif\ {#1 }\ \ttthen\  {#2}\ \ttelse\ {#3}}}
\newcommand{\LET}[3]{{\ttlet\ {#1}\ =\ {#2}\ \ttin\ {#3}}}
\newcommand{\FLET}[3]{{\ttletf\ {#1}\ =\ {#2}\ \ttin\ {#3}}}
\newcommand{\ULET}[3]{\ttletu\ {#1}\ =\ \ttunfold\ {#2}\ \ttin\ \ {#3}}

\newcommand{\ttfold}{\mathtt{fold}}
\newcommand{\ttunfold}{\mathtt{unfold}}
\newcommand{\INS}[4]{\ttletu\ {#1}\ =\ [\ttunfold\ {#2}]\ {#3}\ \ttin\ {#4}}
\newcommand{\GEN}[1]{[\ttfold\ {#1}]}
%\newcommand{\rloc}{\ensuremath{r}}
%\newcommand{\loc}{\ell}
\newcommand{\GET}[1]{\mathtt{*}{#1}}
\newcommand{\SET}[2]{\mathtt{*}{#1}\ {:=} \ {#2}}

\newcommand{\ABS}[1]{\tilde{#1}}
\newcommand{\CNC}[2]{{#1}_{#2}}
\newcommand{\typv}{{\alpha}}
\newcommand{\locv}{{\rho}}
\newcommand{\ind}{i}


\newcommand{\VALIDIMP}[3]{{\mathsf{Valid}}(\dbrkts{#1} \wedge \dbrkts{#2} \Rightarrow \dbrkts{#3})}
\newcommand{\irname}[1]{\textsc{[{#1}]}}
\newcommand{\NONNULL}[1]{{#1} \not = 0}
\newcommand{\VALIDPTR}[1]{\mathit{Safe}({#1})}
\newcommand{\SIZEOF}[1]{\ensuremath{\operatorname{sizeof}({#1})}}
\newcommand{\PTRPLUS}[3]{\mathit{PAdd}({#1}, {#2}, {#3})}
\newcommand{\BLKSTART}[1]{\mathit{BS}({#1})}
\newcommand{\BLKEND}[1]{\mathit{BE}({#1})}
\newcommand{\BLKLEN}[2]{\ensuremath{\mathit{BLen}({#1}, {#2})}}
\newcommand{\BLKLENN}{\ensuremath{\mathit{BLen}}}


%%%% Type Checking

%% Misc
\newcommand{\emp}{{\mathtt{emp}}}
\newcommand{\emb}[1]{\dbrkts{#1}}
%\newcommand{\ttsome}[1]{{\mathtt{Some}\ {#1}}}
%\newcommand{\ttnone}{{\mathtt{None}}}
\newcommand{\myfun}[3]{{\ftyp{#1}{#2} \rightarrow {#3}}}
%%\newcommand\UNFOLD[2]{\SUBST{#1}{t}{#2}}
\newcommand{\hastype}{:}
\newcommand{\tcons}[2]{\mathtt{C}_{#1}{#2}}

\newcommand{\falset}[1]{\overline{#1}}
\newcommand{\mybar}[1]{\zug{#1}}
%\newcommand{\myseq}[1]{\overrightarrow{#1}}
\newcommand{\myseq}[1]{{#1}\ldots}
%\newcommand{\myseq}[1]{\mybar{#1}}
\newcommand{\OFFVAR}[1]{\mathtt{@}{#1}}

\newcommand{\defn}{\ensuremath{\mathtt{define\  }\xspace}}
\newcommand{\eufa}{\ensuremath{\mathtt{EUFA}}}


%%% Subtyping

%\newcommand{\subidx}{\ensuremath{\sqsubseteq}}
\def\subt{\ensuremath{<:}}

%% Judgements 
\newcommand{\inhp}[2]{{#1}/{#2}}
\newcommand{\deriv}{\vdash}
\newcommand{\derivh}{\vdash_h}
\newcommand{\derivl}{\vdash_{\quals}}
\newcommand{\derivml}{\vdash_{ML}}
\newcommand{\sto}{\rho}
\newcommand{\toolname}{\textsc{CSolve}\xspace}
\newcommand{\typesys}{\textsc{Ltll}\xspace}

%% Effect-specific judgements
\newcommand{\ineff}[2]{\inhp{#1}{#2}}
\newcommand{\effaxiomyes}[3]{\forall #1.(#2\wedge #3 \implies \bot)}
\newcommand{\effaxiomno}[3]{\forall #1.(#2\wedge #3 \implies \top)}



%% Types
%\newcommand{\pliqs}{P}
%\newcommand{\aliqs}{A}
\newcommand{\tbas}{\tau}
\newcommand{\tliqs}{\mvreftyp}

%\newcommand{\pliq}{\hat{\pliqs}}
\newcommand{\tliq}{\hat{\tliqs}}
\newcommand{\hpl}{\hat{h}}
\newcommand{\smeta}{\mathbb{S}}
\newcommand{\styp}{\sigma}
\newcommand{\stliqs}{S}
\newcommand{\stliq}{\hat{\stliqs}}
\newcommand{\stliqp}{\tilde{\stliqs}}
\newcommand{\tys}[2]{\inhp{\pliqs_{#1}^{#2}}{{h_{#1}^{#2}}}}

\newcommand{\qexp}[2]{[{#1}]{#2}}
\newcommand{\qtyp}[2]{\forall {#1}.{#2}}
\newcommand{\qtyps}[3]{\qtyp{{#1}, \dots, {#2}}{#3}}
\newcommand{\ftyp}[2]{{{#1}\!:\!{#2}}}
\newcommand{\SUBST}[3]{{#1}[{#2} \mapsto {#3}]}

\newcommand{\kvar}{\kappa}
\newcommand{\tyB}{B}
\newcommand{\tyQ}{Q}
\newcommand{\tyE}{E}
\newcommand{\qs}{{qs}}
\newcommand{\quals}{\mathbb{Q}}
\newcommand{\qualstar}{\quals^\star}
%\newcommand{\vars}{\mathbb{X}}
\newcommand{\consts}{\mathbb{C}}
\newcommand{\kvars}{\mathbb{K}}

%%% Function Signatures
\newcommand{\FSIG}[6]{\qtyp{#1}{\inhp{#2}{#3} \ttarr \inworld{#4}{#5}{#6}}}
\newcommand{\FSIGNOEFF}[5]{\qtyp{#1}{\inhp{#2}{#3} \ttarr \inhp{#4}{#5}}}
\newcommand{\FSIGSMALL}[6]{\qtyp{#1}{\inhp{#2}{#3} \ttarr \inworld{#4}{#5}{#6}}}
\newcommand{\FSIGNOQ}[6]{{\inworld{#1}{#2}{#3} \ttarr \inworld{#4}{#5}{#6}}}


%% Effect-specific types
\newcommand{\eff}{\mveffect}
\newcommand{\effl}{\hat{\mveffect}}
\newcommand{\btwn}[3]{\{#1\leq #2 < #3\}}

%% Operations on effects
\newcommand{\effpar}{\eseq}
\newcommand{\effseq}{\circ}
\newcommand{\effalso}{\otimes}
\newcommand{\effsumop}{\effpar}
\newcommand{\effsum}[2]{#1 \effsumop #2}
\newcommand{\effseqsum}[2]{#1 \effseq #2}
\newcommand{\effprod}[2]{#1 \effalso #2}
\newcommand{\effcheckop}{OK}
\newcommand{\opeffchecksafe}{Safe}
\newcommand{\effchecksafe}[1]{\opeffchecksafe(#1)}
\newcommand{\effcheck}[2]{\effcheckop(#1, #2)}
\newcommand{\effembed}[1]{\dbrkts{#1}}
\newcommand{\effax}{\sigma}
\newcommand{\effvar}{\mveffectname}

% DEPRECATED: USE MVEFFECT* INSTEAD
\newcommand{\efflib}{\mvcommuteset}
\newcommand{\effset}{\mveffectset}

\newcommand{\cartprod}[2]{{#1}\times{#2}}

%%% Effect blocks
\newcommand{\eblck}{p}
\newcommand{\eblckl}{\hat{\eblck}}


%%% Blocks
\newcommand{\blck}{\mvblock}
\newcommand{\blckl}{\hat{\mvblock}}
\newcommand{\hp}{h}
\newcommand{\lmap}{\ensuremath{\gamma}}
\newcommand{\lmapwf}[3]{\ensuremath{{#2} \mapsto {#3} \deriv {#1}}}
\newcommand{\abswf}{\deriv_A}
\newcommand{\cncwf}{\deriv_C}

%\newcommand{\block}{\ensuremath{\beta}}
\newcommand{\singint}[2]{\ensuremath{\langle{#1}\rangle_{#2}}}
\newcommand{\ttrefname}{\mathtt{ref}}
\newcommand{\sref}[1]{\ensuremath{\operatorname{\ttrefname} ({#1})}}
\newcommand{\tref}[2]{\ensuremath{\operatorname{\ttrefname} ({#1}, {#2})}}
\newcommand{\emptyblock}[1]{\ensuremath{\epsilon^{#1}}}



%% Environments
\newcommand{\genv}{\Phi}
\newcommand{\lenv}{\ctx}
\newcommand{\fenv}{\genv}

\newcommand{\EXT}[2]{{#1;\!#2}}
\newcommand{\EXTT}[3]{\EXT{\EXT{#1}{#2}}{#3}}
\newcommand{\EXTTT}[4]{\EXT{\EXT{\EXT{#1}{#2}}{#3}}{#4}}
\newcommand{\UPD}[3]{{#1}[{#2} \mapsto {#3}]}
\newcommand{\GUPD}[2]{\EXT{{#1}}{\langle{#2}\rangle}}
\newcommand{\SOLUPD}[3]{{\mathsf{SolUpd}}({#1},{#2},{#3})}
\newcommand{\remap}[3]{\ensuremath{{#1}[{#2} \mapsto {#3}]}}
\newcommand{\ty}{\mathit{ty}}
\newcommand{\recty}{\mathit{rty}}

%% Typing
\newcommand{\phastyp}[3]{{#1} \deriv {#2} : {#3}}
\newcommand{\pwf}[2]{{#1} \deriv {#2}}
\newcommand{\twf}[2]{{#1} \deriv {#2}}
\newcommand{\abwf}[3]{{#1}, {#2} \deriv_{\mvaloc} {#3}}
\newcommand{\cbwf}[3]{{#1}, {#2} \deriv_{\mvcloc{j}} {#3}}
\newcommand{\hwf}[2]{{#1} \deriv {#2}}
\newcommand{\ewf}[3]{{#1}, {#2} \deriv {#3}}
\newcommand{\wwf}[4]{{#1} \deriv \inworld{#2}{#3}{#4}}
\newcommand{\fwf}[1]{\deriv {#1}}
\newcommand{\sty}[3]{{#1} \deriv {#2} \subt {#3}}
\newcommand{\bst}[3]{{#1} \deriv {#2} \subt {#3}}
\newcommand{\hst}[3]{{#1} \deriv {#2} \subt {#3}}
\newcommand{\est}[3]{{#1} \deriv {#2} \subt {#3}}
\newcommand{\wst}[3]{{#1} \deriv {#2} \subt {#3}}

%% Heap-related predicates

\newcommand{\opname}[1]{\ensuremath{\mathrm{#1}}\xspace}

\newcommand{\opbbegin}{\opname{BB}}
\newcommand{\bbegin}[1]{\ensuremath{\opbbegin({#1})}}

\newcommand{\opread}{\opname{Read}}
\newcommand{\eread}[1]{\ensuremath{\opread({#1})}}

\newcommand{\opwrite}{\opname{Write}}
\newcommand{\ewrite}[1]{\ensuremath{\opwrite({#1})}}

\newcommand{\opaccumulate}{\opname{Accumulate}}
\newcommand{\eaccumulate}[1]{\ensuremath{\opaccumulate({#1})}}

\newcommand{\opcheck}{\opname{Check}}
\newcommand{\echeck}[1]{\ensuremath{\opcheck({#1})}}


%% Effect Operators

\newcommand{\opefflookup}{\ensuremath{\opname{LU}}}
\newcommand{\efflookup}[2]{\opefflookup(#1, #2)}


%% Evaluation

\newcommand{\memsafety}{\ttname{Mem}}
\newcommand{\determinism}{\ttname{Det}}
\newcommand{\chk}{\checkmark}
\newcommand{\ttmerge}{\ttname{Merge}}
\newcommand{\ttseqmerge}{\ttname{Seq\_Merge}}
\newcommand{\tta}{\ttname{a}}
\newcommand{\ttb}{\ttname{b}}
\newcommand{\ttc}{\ttname{c}}
\newcommand{\DPJ}{\textsc{DPJ}\xspace}


==> return.tex <==
By \cref{l:exprtypelemma},
%
\[
\denotef{\ctx}{\heap} =
  \exquant{\ldots}G \hpjoin H_{\loc_0} \hpjoin \cdots \hpjoin  H_{\loc_n}
\]
%
Applying the frame rule to the proof rule for \returnName, our consequence
is
%
\[
\exquant{x_r}(x_r = e)\hpjoin
  \exquant{\ldots}G \hpjoin H_{\loc_0} \hpjoin \cdots \hpjoin  H_{\loc_n}
\]
%
Which trivially satisifies the empty world $\denote{\emptyset} \myeq \top$.
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "proof_main.tex"
%%% End: 


==> return_fundef.tex <==
% \begin{lemma}\label{l:return}
\showreturnlemma
% \end{lemma}
\begin{proof}
By inversion on the judgement, we must have typed a
statement $s' = \return{e}$ for some expression, or a sequence
of statements ending in a \returnName.
%
Without loss of generality, we assume that $s$ is a single
\returnName statement. (The proof for a sequence of statements
is the same).
%
Applying the frame rule,
we derive the following for \returnName:
%
\[ \htriplec{ \denotef{\ctx}{\heap\hpjoin\heap'} }
            { \return{e} }
            { \denotef{\ctx}{\heap\hpjoin\heap'} 
              \wedge \exquant{x_\retId}(x_\retId = e) }
\]
%
By hypothesis and \cref{l:subtyping} the following facts hold:
%
\begin{align*}
\denote{\ctx} & \Rightarrow \sprop{\sub{x_\retId}{e}\ty_\retId}{e}\\
\denotef{\ctx}{\heap} & \Rightarrow \denotef{\ctx}{\sub{x_\retId}{e}\heap_\retId}
\end{align*}
%
and thus
%
\[ \htriplec{ \denotef{\ctx}{\heap\hpjoin\heap'} }
            { \return{e} }
            { \exquant{x_\retId}\denotef{\tybind{x_\retId}{\ty_\retId}}{\heap_\retId} }
\]
\end{proof}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "proof_main.tex"
%%% End: 


==> sep.tex <==
% type C[α] = ∃! H . T
% C =

((l ↦ C * r ↦ C) -* C)

% ∃ l r. C ∧ p ↦ T

% function foo :: ∀α. ∀l. (<x>+null)/l ↦ α ⇒ ∃m. <m>/m ↦ α


==> seplang.tex <==
\begin{figure}
\judgementHead{Proof Rules}{\htriplec{P}{c}{Q}}
$$
\inference{
}{
  \htriple{\hpemp}
          {\evar = \alloc{\many{\field:\expr}}}
          {\sepmap{\mcode{x}}{\many{\field:\expr}}}
}
$$

$$
\inference{
}{
  \htriple{\sepmap{\evar}{\sepfld{\field}{-}}}
          {\access{\evar}{\field} = \expr}
          {\sepmap{\evar}{\sepfld{\field}{\expr}}}
}
$$

$$
\inference{
  \shtapp{\pred}{\loc}{\evar} \myeq \equant{\many{z}}T
  \\
  \theta = \sub{\many{z}}{\many{z'}}\quad \many{z'}\mbox{ do not appear free in }P
}{
  \htriple{\shtapp{\pred}{\loc}{\evar}}
          {\unwind{\loc}}
          {\theta T}
}
$$

$$
\inference{
  \shtapp{\pred}{\loc}{\evar} \myeq \equant{\many{z}}T
  \\
}{
  \htriple
    {T}
    {\wind{\loc}}
    {\shtapp{\pred}{\loc}{\evar}}
}
$$

$$
\inference{
}{
  \htriple
    {\sepmap{\loc}{\evar}}
    {\conc{\loc}}
    {\sepmap{\loc}{\evar}}
}
$$
\caption{Proof rules for \lang statements}
\end{figure}

%%% Local Variables: 
%%% mode: latex
%%% eval: (TeX-PDF-mode 1)
%%% TeX-master: "main.tex"
%%% End: 


==> shape.tex <==
\section{Shape Analysis}\label{sec:shape}

The use of the alias type discipline, in which each heap binding
denotes 0 or 1 singleton run-time values, allows \toolname
to handle the problems of materializing, summarizing, and joining
heap shapes in a straightforward manner. 
%
These problems are solved syntactically, using logical information from
the refinement type system to compute precise summaries.
%
The heap \emph{fold} and \emph{unfold} operations are the 
backbone of \toolname's type system; they provide the anchors 
at which the type system respectively \emph{generalizes} 
and \emph{instantiates} facts about linked structures.
%
In this section we explicate these concepts.


\mypara{Materialization}
%
A linked data structure such as a list is a collection of cells rooted
at some location $\loc$.
%
Thus, to inspect the nodes that comprise a structure, the root must
first be \emph{unfolded} -- 
which is exactly the function of the heap annotation $\unwind{\loc}$.
%
As the application $\tyapp{\tycon}{\tvar}$ is a summary of the data
structure denoted by $\tycon$, unfolding a location containing an
application of $\tycon$, yields \emph{unique} heap cells in addition
to summaries of the remainder of the data structure.

\mypara{Summarization}
%
Likewise, to build a new collection of cells rooted at $\loc$, 
a summary of the data structure must be constructed, which is the
purpose of the $\wind{\loc}$ annotation.
%
Building a summary of a data structure entails checking that the
contents of the data structure all satisfy the data structure's
invariants.
%
Precision is easily lost in this step: a sound type checker must be
conservative and ensure that each possibly-reachable location satisfy
the necessary invariants.
%
In \cref{sec:check} we saw that heap folding uses environment
guards to reason about reachability, crucially restricting
subtyping to the reachable heap.
%
In this way, we connect the alias and refinement type systems: we
exploit precise logical invariants to determine which pointers are
\vnull, and hence which locations are reachable.

\mypara{Control Flow Joins}
%
\abakst{we added the pad statement just before the POPL Deadline --
  maybe we should discuss it?}
%
After type checking the ``then'' and ``else'' branches of a
conditional, the rule \rtite must \emph{join} the resulting
environments, necessarily joining the heaps from the two branches.
%
With the heaps in both branches folded up, \rtite checks that each
branch's heap ($\heap_1$ and $\heap_2$) is a subheap of $\heap'$.
%
This requirement critically entails 
\begin{inparaenum}[(1)]
  \item
    $\heap_1$ and $\heap_2$ both contain at least the locations in $\heap'$ 
    and
  \item
    the types at these locations have the same \emph{base} type, effectively
    ensuring that the shape of the heap matches at each location.
\end{inparaenum}
% 
Furthermore, the invariants at each location in the joined heap
must be implied by the invariants at the corresponding locations
in $\heap_1$ and $\heap_2$.
%
Because data structure invariants are expressed as types, the natural
least upper bound is expressed as the disjunction of the invariants
from both branches.
%
Thus, the problem of joining heap summaries is simply reduced to heap
subtyping.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End: 


==> shape2.tex <==
\section{Discussion: Type-based Shape Analysis} \label{sec:shape}

\toolname is a syntax-directed means of doing \emph{shape analysis},
\ie of precisely tracking invariants about linked structures on the
heap.  Shape analysis is a challenging problem that has been addressed
by a variety of techniques over the last few decades.
%
Any solution must tackle three related sub-problems.
%
First, how to \emph{represent} an unbounded collection of cells,
while retaining tractability and precision.
%
Second, how to \emph{instantiate}
the properties of a collection, thus obtaining properties
of a particular element.
%
Third, how to \emph{generalize}
individual cells into properties of the collection.
%
We discuss \toolname's approach in this section.

\mypara{Deep Factorization}
%
The most important aspect of \toolname is its
\emph{deep factorization} of the representation
and analysis into \emph{physical}
and \emph{logical} components.
%
It is standard for SL based analyses to partition
the representation into a form $\Pi \wedge \Sigma$
where, quoting \cite{berdine2006smallfoot}
  ``$\Pi$ is a pure boolean condition and $\Sigma$
    is a \verb+*+ combination of heap predicates''
which
  ``enables a symbolic execution mechanism.''
%
This form of partitioning is analagous to the
environment-and-heap representation (via $\Gamma / \Sigma$)
of alias typing and \toolname:
%
the syntax of the program logic separates
assertions about immutable scalars from
assertions about the heap.

In contrast, by deep factorization we mean that properties about
\emph{heap structures} are represented by composing a ``physical''
alias type that only tracks links, with a ``logical'' refinement that
captures semantic properties.
%
To describe a list of natural numbers
in SL, we would write a variant of the
list-segment predicate that conjoins each
datum to be non-negative, yielding a monolithic
representation that conflates the physical links with
the logical data property. (One could parameterize the
@lseg@ predicate with a property, but that leads to
higher-order specifications, requiring manual proof
\cite{HTT}.)
In \toolname, the type
$\tlist{\tnat}$ composes the alias type
describing lists with a simple refinement describing each cell.

\mypara{Representation}
%
Deep factorization allows us to refine alias types
with logical refinements that are precise enough
to prove functional correctness properties.
%
In contrast with previous SL based analyses \toolname
does not require built-in
recursive predicates (\eg list-segments)
that represent collections.
%
In contrast with abstract-interpretation based
analyses~\cite{TVLA}, \toolname does not require
(instrumentation) predicates that are used
to partition the heap into independent collections.
%
Type definitions in \toolname define the analog of recursive
predicates that represent collections, while alias typing isolates
independent collections of values.

\mypara{Instantiation}
%
Facts about collections are
instantiated or materialized at @unfold@ sites.
%
This yields two concrete benefits over other shape analyses.
%
First, it is trivial to determine \emph{where} to unfold:
prior to field accesses, analogous to unfolding at pattern-matching
sites in functional languages.
%
Second, the algorithm for materialization directly follows from the
classical unfolding of recursive types.

\mypara{Generalization}
%
\toolname performs
generalization (or summarization) -- in two steps:
%
(1)~a @fold@ operation, the dual of @unfold@, which
    packs a concrete cell back into a collection
    (making it inaccessible until a subsequent unfold),
    and
%
(2)~a heap subtyping operation, that checks that
    the refinements of the folded (or summarized)
    structure, soundly overapproximate
    those of the individual cells comprising the structure.
%
This approach offers a crucial advantage over prior analyses:
we do not require structure- or property- specific
abstract domains or widening algorithms.
%
Instead, types provide an abstract domain for collections,
and quantifer-free refinements provide a domain for logical
properties.
%
The physical type system makes it trivial to identify @fold@
locations -- namely control-flow joins where the heaps
do not match up.
%
Factorization reduces ``global'' subsumption (or joins) to
simple ``local'' implications that are automatically discharged by SMT
solvers.

%%% CUT for VMCAI \mypara{Challenges}
%%% CUT for VMCAI %
%%% CUT for VMCAI To faithfully represent idiomatic pointer manipulating programs,
%%% CUT for VMCAI types like $\tlist{A}$ should represent lists with \emph{zero or more}
%%% CUT for VMCAI elements.
%%% CUT for VMCAI %
%%% CUT for VMCAI In SL this is represented by a disjunction in the
%%% CUT for VMCAI list-segment predicate -- either the pointer is \vnull
%%% CUT for VMCAI \emph{or} it refers to a cell with a next field that
%%% CUT for VMCAI is also a list -- and one can use the full program
%%% CUT for VMCAI logic and explicit semantic non-\vnull tests to
%%% CUT for VMCAI determine which of the two cases hold.
%%% CUT for VMCAI %
%%% CUT for VMCAI However, to reason about this disjunction in a purely
%%% CUT for VMCAI syntactic fashion -- via alias typing -- we require
%%% CUT for VMCAI tagged unions and pattern matching, which is not
%%% CUT for VMCAI idiomatic in pointer manipulating programs.
%%% CUT for VMCAI
%%% CUT for VMCAI This problem is solved by delegating the
%%% CUT for VMCAI reasoning about zero-or-more elements to the
%%% CUT for VMCAI \emph{refinement} system.
%%% CUT for VMCAI %
%%% CUT for VMCAI We check that each dereferenced pointer enjoys the refinement ${\vv
  %%% CUT for VMCAI \neq \vnull}$, \ie is a non-null pointer.
%%% CUT for VMCAI %
%%% CUT for VMCAI To allow an \emph{empty} collection
%%% CUT for VMCAI of one type to be subsumed by a collection
%%% CUT for VMCAI of a different type, \eg to fold an empty tail list
%%% CUT for VMCAI of type $\tlist{p}$ into a list of type $\tlist{q}$
%%% CUT for VMCAI we guard the sub-typing check
%%% CUT for VMCAI with the condition that the collection pointer be non-null.
%%% CUT for VMCAI %
%%% CUT for VMCAI This is the mechanism used to perform the fold in the \emph{then}
%%% CUT for VMCAI branch in \cref{fig:ex3}.
%%% CUT for VMCAI
%%% CUT for VMCAI This approach prevents unreachable cells from weakening
%%% CUT for VMCAI the invariants of a collection, allowing for ``strong updates.''
%%% CUT for VMCAI %
%%% CUT for VMCAI Interactions between
%%% CUT for VMCAI the physical and logical analyses are reduced to non-null checks
%%% CUT for VMCAI that are placed by the alias type system and
%%% CUT for VMCAI discharged by the refinement type system.

\mypara{Limitations}
While factoring allows \toolname to precisely
and automatically verify properties of a variety
of structures, it is restricted to programs
that adhere to a certain typing discipline.
%
Intuitively \toolname is limited to ``tree-like''
ownership structures: while sharing and cycles
are allowed (as in double- or cyclic-lists),
there is a tree-like \emph{backbone} used
for traversal.
%
For example, even with a singly linked list,
our system will reject programs that traverse
deep into the list, and return a pointer to a
cell \emph{unboundedly} deep inside the list.
%
We believe it is possible to exploit the connection
made between the SL notion of ``magic wands" and
the type-theoretic notion of ``zippers" \cite{Huet97}
identified in \cite{summersECOOP15} to enrich the
alias typing discipline to accommodate such access patterns.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> soundness.tex <==
\section{Soundness}\label{sec:soundness}

The constraints output by \fn{CGen} enjoy the
following property. 
%
Let ($C$,$\ctx'$,$\heap'$) be the output of 
\inline{CGen($\Phi$,$\ctx$,$\heap$,s)}.
%
If $C$ is satisfiable, then there exists some solution $K$ such that
$\stmttype{K\ctx}{K\heap}{\stmt}{K\ctx'}{K\heap'}$\cite{LiquidPLDI08},
\ie there is a type derivation using the refinements from $K$.

We translate types, environments and heaps into separation logic
\emph{assertions} and hence, typing derivations into 
\emph{proofs}. 
%
\begin{figure}[tb]{\small
\begin{align*}
\sbase{\reftt{\tnull}}{\evar} & \myeq (\evar = \vnull) \wedge \sub{\vv}{\evar}\pred\\
\sbase{\reftt{\tref{\loc}}}{\evar} & \myeq ((\evar = \loc) \wedge (\evar \neq \vnull)) \wedge \sub{\vv}{\evar}\pred\\
\sbase{\reftt{\trefm{\loc}}}{\evar} & \myeq
  (\sbase{\tref\loc}{\evar} \vee \sbase{\tnull}{\evar})\wedge \sub{\vv}{\evar}\pred\\
  \shprop{\reftt{\tyapp{\tycon}{\ty}}}{\loc}{x} & \myeq
  ((\loc \neq \vnull) \Rightarrow (\sprop{\reftt{\tyapp{\tycon}{\ty}}}{x}) \hpjoin \shtapp{\ty}{\loc}{\evar})
  \\
  & \wedge\ ((\loc = \vnull) \Rightarrow (x = \vnull))\\
    \denotef{\ctx}{\heap} & \myeq
    %\exquant{(\fv{\ctx}\cup\fv{\heap})} 
      \bigwedge\limits_{{\expr \in \ctx}} \expr
      \bigwedge\limits_{{\tybind{\evar}{\ty} \in \ctx}}  \sprop{\ty}{\evar}
    \wedge
      \bigast\limits_{\hplocty{\loc}{x}{\ty} \in \heap} 
      \shprop{\ty}{\loc}{x}
\end{align*}
}%
\caption{Translations of selected types}
\label{fig:semfig}
\end{figure}
%
\cref{fig:semfig} gives some examples of our translation.
%
\shtapp{\ty}{\loc}{\evar} denotes a predicate derived from a type definition. 
%
For example, the corresponding list predicate would be defined:
\begin{align*}
  \seplista{A}{\loc}{x}  \doteq
      & \ \sepunfold{\loc}{x} \wedge
      \exquant{h, t, \loc_t} \headlista{A}{\loc}{h}{\loc_t} \hpjoin 
      ((\loc_t \neq \vnull) \Rightarrow \seplista{A}{\loc_t}{t}) \\
  \headlista{A}{\loc}{h}{\loc_t} \doteq 
      & \  \denote{\hplocty{\loc}{h}{\tobj{\tybind{\fn{data}}{A}
                                          ,\tybind{\fn{next}}{\trefm{\loc_t}}}}
                  } 
\end{align*}
%
The predicate $\sepunfold{\loc}{x}$ ``unpacks'' the snapshot $x$ into
a separation logic heap assertion that characterizes heaps where $x$
is the snapshot at $\loc$.

We prove the following theorems: 
\showstmtprocthm
$\Pre{\funschema}$, $\Post{\funschema}$ and $\Body{f}$ are the translations
of the input and output types of the function, the function (body) statement.
%
As a corollary of this theorem, our main soundness result follows:
%
\showtypeproofs
%
If we typecheck a program in the empty environment, we get a valid 
separation logic proof of the program starting with the pre-condition \ttrue.
%
We can encode programmer-specified \code{assert}s as calls to a special 
function whose type encodes the assertion. 
%
Thus, the soundness result says that if a program typechecks then on
\emph{all} executions of the program, starting from \emph{any} input
state:
%
\begin{inparaenum}[(1)]
  \item all memory accesses occur on \nnull pointers, and
  \item all assertions succeed.
\end{inparaenum}
%

The soundness proof proceeds by induction on the typing derivation. 
We show that the typing rules correspond to separation logic proofs
using the appropriate proof rule; see~\cref{sec:proof} for details.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End: 


==> soundness2.tex <==

% Translation
%   Examples
%   Theorem: Statement & Procedure Folding
%   Corollary: Soundness

% Folding & Measures
%   Examples
%   Lemma: Folding 

% Subtyping
%   Lemma: Subtyping

\section{Soundness}\label{sec:soundness}

We prove that \toolname{}'s type system is sound by translating 
types, environments and heaps into separation logic \emph{assertions}
and hence, typing derivations into separation logic \emph{proofs}.
Next, we illustrate the translation by example and present the 
key theorems; deferring to \S~\ref{sec:proof} for details.

\subsection{Translation}

We define a translation $\denote{\cdot}$ (\S~\ref{sec:defs}) 
from types, contexts, heaps, and judgements to assertions 
in separation logic. 
%
We translate a typing context $\ctx,\heap$ by conjoining the 
translations of $\ctx$ and $\heap$, \ie 
%
$$\denotef{\ctx}{\heap} \doteq \ \denote{\ctx}\wedge \denote{\heap}$$
%
Next, we illustrate the translation of local contexts $\ctx$ 
and heaps $\heap$ using the \code{insert} function from \Cref{fig:ex4}.

\mypara{Local Contexts}
%
We translate local contexts $\ctx$ into a conjunction of 
\emph{pure}, \ie heap independent, assertions over the 
binders in $\ctx$.
%
The type context $\ctx_1$ at \cref{line:ex4start} contains
two assumptions:
%
\begin{align*}
\ctx_1 \doteq & \ \tb{\x}{?\tref{\addr{\x}}},\ \isnull{\x} \\
%
\intertext{which respectively state that \x is a possibly \vnull 
reference \addr{\x}, and a guard that \x is definitely \vnull.
Note that \addr{\x} \emph{does not} denote the application of 
a function called \addr{}; it is a distinct heap location 
\emph{named} \addr{\x}. 
We translate $\ctx_1$ by conjoining the results of translating its
constituent assumptions:} 
%
\denote{\ctx_1} \doteq & \ (\x \neq \vnull \Rightarrow \x = \addr{\x}) \wedge (\x = \vnull)
%
\end{align*}
%
Note that translation states that if \x is not \vnull, then \x refers
to a valid heap location as \addr{\x} is also not \vnull.

\mypara{Heaps: Recursive Structures}
%
We interpret heaps as (separated) conjunctions of \emph{impure} 
(\ie, heap-dependent assertions) and \emph{pure} assertions 
corresponding to the types of the values stored in each location.
%
To faithfully model \vnull terminated recursive structures 
(\eg the case where a list is empty) each location in $\dom{\heap}$ 
may be $\vnull$.
%
Thus, the heap at \cref{line:ex4start}, and its interpretation are
%
\begin{align}
  \heap_1         \doteq  & \ \hb{\x}{\tb{\x_0}{\tlist{A}}} \notag \\
% \intertext{is interpreted as the assertion} 
\denote{\heap_1}  \doteq  & \ (\addr{\x} \neq \vnull) \Rightarrow \seplista{A}{\addr{\x}}{\x_0}
 \label{eq:trans:heap1}
\end{align}
%
stating that if the location exists on the heap, 
\ie is non-\vnull, then it refers a \emph{valid list}, described 
by a \emph{predicate} in separation logic.


\mypara{Type Predicates}
%
We translate the definition of the $\tlist{A}$ type into 
a (separation logic) type predicate that characterizes the
part of the heap where a $\tlist{A}$ is stored.
%
For example, for the list type from \cref{fig:ex4} we define 
the type predicate as:
%%
\begin{align*}
  \seplista{A}{\loc}{x}  \doteq
      & \ \sepunfold{\loc}{x} \wedge
      \ \exquant{h, t, \loc_t} \headlista{A}{\loc}{h}{\loc_t} \hpjoin 
                                  \seplista{A}{\loc_t}{t} \\
  \headlista{A}{\loc}{h}{\loc_t} \doteq 
      & \  \denote{\hplocty{\loc}{h}{\tobj{\tybind{\fn{data}}{A}
                                          ,\tybind{\fn{next}}{\trefm{\loc_t}}}}
                  } 
\end{align*}
%
Intuitively, the conjuncts of the assertion $\seplista{A}{\loc}{x}$ say:
%
\begin{inparaenum}[(1)]
  \item the snapshot $x$ is a \emph{pure value} comprising all the 
        records (data and references) that are transitively reachable 
        on the heap, starting at the root, $\loc$, and
  \item the heap satisfies the ``shape" invariants defined by the recursive
        alias type \tlist{A}
\end{inparaenum}
%        
That is, the assertion $\seplista{A}{\loc}{x}$ states that the snapshot 
$x$ corresponds to the heap structure rooted at $\loc$ on the heap.
%
We prove (\S~\ref{sec:proof}) that each well-formed type definition can be 
translated into a type predicate analagous to the above, which lets
us translate all heap-locations mapped to recursive types in a manner
analagous to~\cref{eq:trans:heap1}.

\mypara{Records} 
%
The other case is for heap-locations that are mapped to plain records.
At \cref{line:ex4fold}, \code{insert} has 
allocated a record to which \y refers.
%
There, the type context and its translation are
\begin{align}
%
\ctx_2 \doteq & \ \ctx_1, \tb{\y}{\addr{\y}} \label{eq:ctx2}\\
%
% \intertext{translates to}
\denote{\ctx_2} \doteq & \denote{\ctx_1} \wedge (y \neq \vnull \Rightarrow y = \addr{y}) \wedge (y \neq \vnull)  \label{eq:ctx2:trans} \\
\intertext{\ie the binding for \y is translated to the assertion for a
maybe-null pointer plus the fact that \y is not-null. The heap at
\cref{line:ex4fold} is}
\heap_2 \doteq & \ \heap_1 \hpjoin \sepmap{\addr{\y}}{y_0} \wedge {y_0 = \tobj{\fld{data}{\code{k}},\fld{next}{\vnull}}} \label{eq:heap2} \\
\intertext{which translates directly into}
\denote{\heap_2} \doteq & \ \denote{\heap_1} \hpjoin (\sepmap{\addr{\y}}{y_0} \wedge {y_0 = \tobj{\fld{data}{\code{k}},\fld{next}{\vnull}}}) \nonumber %\label{eq:heap2:trans}
\end{align}
%
\ie we interpret the binding as a separation logic
assertion \cite{Reynolds02}.

\subsection{Soundness Theorem}
%
We use the above translations to state and prove soundness by showing that
a valid typing of a statement \stmt under given contexts can be translated 
into a valid separation logic proof of \stmt under pre- and post-conditions 
obtained by translating the contexts.

\showstmtprocthm

By virtue of how contexts are translated, the result of the translation is 
\emph{not} a vacuous separation logic proof (\ie one beginning starting with 
the precondition $\mathit{false}$). 
%
As a corollary of this theorem (and the
definition of \denote{\cdot}) our main soundness result follows:

\showtypeproofs

That is, if we typecheck a program in the empty environment, we get a valid 
separation logic proof of the program starting with the pre-condition \ttrue.
%
We can encode programmer-specified \code{assert}s as calls to a special 
function that \emph{requires} the argument \ttrue. Thus, the soundness result 
says that if a program typechecks then on \emph{all} executions of the program, 
starting from \emph{any} input state:
%
\begin{inparaenum}[(1)]
  \item all memory accesses occur on \nnull pointers, \ie every access is safe, 
  \item all assertions succeed.
\end{inparaenum}

We prove the typing theorem by induction on the typing derivation. 
We show that the typing rules for statements can be
translated into the appropriate separation logic proof rules.
%
The most critical parts of the proof are translating the rules for 
\emph{folding} (and unfolding) recursive type definitions, and 
\emph{subtyping}. 
%
We prove that our folding and subtyping judgments can be translated to
entailments in separation logic, by showing that:

\showfolding

\showsubtyping

We use the above lemmas to translate the (occurrences of) 
%
subtyping,
%
heap subtyping, and
%
heap folding 
%
judgments (from \cref{fig:subtyping} and \cref{fig:heapfolding})
into separation entailments, thereby allowing us 
to translate the rules for \windName, \unwindName and subtyping 
into a combination of ``skip" statements and the consequence rule 
of separation logic.

For example, at \cref{line:ex4fold}, \code{insert} is about to 
return the list that \y points to (at location \addr{\y}). 
%
At this point the context is given by the $\ctx_2$ 
and $\heap_2$ from \cref{eq:ctx2} and \cref{eq:heap2}. 
%
\toolname checks that the context satisfies the output type of 
\code{insert} \ie that \addr{\y} is the root of a valid list whose 
length equals one greater than (the snapshot of) the input \x.
%
To do so, it uses the subtyping rules and \rtwind to obtain 
the following context at \cref{line:ex4return}: 
%
\begin{align}
\ctx_3  & \doteq \ \ctx_2, \mlen{y_1} = 1 + \mlen{\vnull} \notag \\
\heap_3 & \doteq \ \heap_1 \hpjoin \hb{\y}{\tb{\y_1}{\tlist{A}}} \notag \\
\intertext{Using \cref{lem:subtyping} and \cref{lem:folding} we have:}
\denotef{\ctx_2}{\heap_2} \Rightarrow & \ \denotef{\ctx_3}{\heap_3} \label{eq:impl23}
\end{align}
%
In particular, note that $\y_1$ names the snapshot value
corresponding to the (single-celled) list referred to by 
\y, and the measure instantiation due to \rtwind states 
that the length of the snapshot is 1 greater than the 
length of the tail \vnull.

The implication \cref{eq:impl23} follows by expanding the 
definitions of the length measure, the snapshot predicate 
and the type predicate. %
%
We can use the implication to translate the type 
checking deduction of \toolname at this point, into an
entailment, and hence, instance of the consequence rule 
in the separation logic.

\subsection{Summary}

Soundness follows by a carefully designing \toolname as 
a restricted and stylized separation logic where the \emph{heavy lifting} 
of reasoning inductively about linked structures is done by the
syntax-directed \emph{decision procedure} of alias typing \cite{AliasTypesRec}. 
%
In particular, we reconcile expressive and automatic verification of 
linked structures by adhering to the following principles:
\abakst{This was enum before! Check?}
% \begin{enumerate}
% \item

 Each data type definition corresponds to an inductively defined
  set of \emph{pure} values.  We interpret these values as
  \emph{snapshots} of a data structure at a particular point in time:
  all of the values stored in the data structure, including internal
  pointers.
  
% \item
 Each heap binder refers to a snapshot value, which lets \toolname 
  soundly refer to \emph{previous} values (snapshots) of a structure 
  inside refinements and thus encode correctness properties as logical 
  predicates about heap binders.
  
% \item 
Alias typing ensures that no member of a structure is modified 
  without first \emph{unfolding} the data structure, at which point 
  fresh names are given to the corresponding heap binders that reflect
  the ``new" snapshots at the location. 
  In other words, the alias type system lets \toolname update the heap 
  binders \emph{locally}, without having to deal with transitive reachability.
% \end{enumerate}
 
Of course, note that the \toolname \emph{does not} actually 
perform the translation \denote{\cdot} (or expand the definitions
of the snapshot or type predicates, or use separation logic 
entailments). We merely use the translation to separation 
logic to prove \toolname sound.


%%%% TMI \subsection{Folding and Subtyping}
%%%% TMI 
%%%% TMI Let us illustrate this using the example from \cref{fig:ex4}.
%%%% TMI At \cref{line:ex4fold}, \code{insert} is about to return the list
%%%% TMI that \y points to (at location \addr{\y}). Recall that at this point
%%%% TMI the context is given by the $\ctx_2$ and $\heap_2$ from \cref{eq:ctx2} 
%%%% TMI and \cref{eq:heap2}. Thus, at this point \toolname checks that \addr{\y} 
%%%% TMI is the root of a valid list whose length equals one greater than 
%%%% TMI (the snapshot of) the input \x.
%%%% TMI 
%%%% TMI The type checking proceeds in two steps. 
%%%% TMI 
%%%% TMI First, we s
%%%% TMI 
%%%% TMI %
%%%% TMI \begin{inparaenum}[(1)]
%%%% TMI   \item 
%%%% TMI     the \code{next} field of $y_0$ is a possibly-\vnull reference to a valid $\tlist{A}$ 
%%%% TMI     whose s
%%%% TMI     %
%%%% TMI   \item \emph{naming} the new $\tlist{A}$ at
%%%% TMI     \addr\y -- \ie, determining the value of the \emph{snapshot}
%%%% TMI     at \addr{\y}
%%%% TMI \end{inparaenum}.
%%%% TMI %
%%%% TMI 
%%%% TMI 
%%%% TMI 
%%%% TMI 
%%%% TMI \begin{verbatim}
%%%% TMI 1. SHOW LEMMA
%%%% TMI 
%%%% TMI 2. At line the rule T-Fold takes us from G1/S1 to G3/S3 
%%%% TMI    in two steps:
%%%% TMI 
%%%% TMI       [G1,S1] --- 1 ---> [G2,S2] 
%%%% TMI       [G2,S2] --- 2 ---> [G3,S3]
%%%% TMI 
%%%% TMI       (1) [[G1, S1]] => [[G2, S2]]
%%%% TMI       (2) [[G2, S2]] => [[G3, S3]]
%%%% TMI 
%%%% TMI    where 
%%%% TMI 
%%%% TMI       (1) is |>                                     ... which is rule of consequence due to lemma
%%%% TMI       (2) is "folding" i.e. rolling up the type def ... which is just by the definition of type predicate
%%%% TMI 
%%%% TMI 
%%%% TMI 3.  (1) is just rule of consequence (thanks to LEMMA),
%%%% TMI     (2) the first of these steps is just consequence
%%%% TMI \end{verbatim}
%%%% TMI %
%%%% TMI In the type system, this corresponds to deriving
%%%% TMI %
%%%% TMI \[
%%%% TMI \heapfoldxy{\ctx_2}
%%%% TMI            {\ty_a}
%%%% TMI            {\hpemp}
%%%% TMI            {\ty_b}
%%%% TMI            {\hplocty{\loc}{t}{\tlist{A}}}
%%%% TMI            {y_0}{y_0}
%%%% TMI \]
%%%% TMI %
%%%% TMI where
%%%% TMI %
%%%% TMI \begin{align*}
%%%% TMI   \ty_a & \doteq {\tobj{\fld{data}{A}, \fld{next}{\tnull}}} &
%%%% TMI   % \heap_a & \doteq
%%%% TMI   % {\hplocty{\addr{\y}}{y_0}{\ty_a}}\\
%%%% TMI   \ty_b & \doteq {\tobj{\fld{data}{A}, \fld{next}{\trefm{\loc}}}}
%%%% TMI   % \heap_b & \doteq
%%%% TMI   % {\hplocty{\addr{\y}}{y_0}{\ty_b}
%%%% TMI   %   \hpjoin \hplocty{\loc}{t}{\tlist{A}}}
%%%% TMI \end{align*}
%%%% TMI %
%%%% TMI Due to our interpretation of type contexts, this judgement
%%%% TMI has the following meaning in separation logic:
%%%% TMI %
%%%% TMI \begin{align*}
%%%% TMI \denotef{\ctx_2}{\hplocty{\addr{\y}}{y_0}{\ty_a}} 
%%%% TMI & \Rightarrow 
%%%% TMI \exquant{\loc,t}
%%%% TMI \denote{\hplocty{\addr{\y}}{y_0}{\ty_b}\hpjoin \hplocty{\loc}{t}{\tlist{A}}}\\
%%%% TMI \denotef{\ctx_2}{\hplocty{\addr{\y}}{y_0}{\ty_a}} 
%%%% TMI & \Rightarrow 
%%%% TMI \exquant{y_1}\sepunfold{\addr{\y}}{y_1}
%%%% TMI \end{align*}
%%%% TMI \abakst{Ditch the exists here?}
%%%% TMI %
%%%% TMI The first implication says that the heap reachable from \addr{\y} in
%%%% TMI fact satisfies the $\tlist{A}$ invariant.
%%%% TMI %
%%%% TMI The second says that the snapshot of the heap at \addr{\y} is the
%%%% TMI \emph{value} named by $y_1$, which in this case happens to be equal to
%%%% TMI $
%%%% TMI \tobj{\fld{data}{e},\ \fld{next}{\vnull}}.
%%%% TMI $
%%%% TMI %
%%%% TMI By the definition of $\fn{list}$, these facts are sufficient to conclude
%%%% TMI \[
%%%% TMI \denotef{\ctx_2}{\heap_2} 
%%%% TMI \Rightarrow  \denote{\ctx_2} 
%%%% TMI      \wedge (\denote{\heap_1} \hpjoin \seplista{A}{\addr{\y}}{y_1}).
%%%% TMI \]
%%%% TMI 
%%%% TMI \mypara{Measures}
%%%% TMI %
%%%% TMI Just as heap binders correspond to snapshots of the heap in our
%%%% TMI interpretation, we interpret measures as functions over these snapshot
%%%% TMI values.
%%%% TMI %
%%%% TMI The measure well-formedness rules ensure that these functions are
%%%% TMI are well-defined.
%%%% TMI %
%%%% TMI %
%%%% TMI Prior to folding up the list at \addr\y, we knew that \code{y.next}
%%%% TMI was equal to \vnull, so by definition $\len(y_1) = 1$, giving us the
%%%% TMI strengthened environment:
%%%% TMI %
%%%% TMI \[
%%%% TMI \denote{\ctx_3} = \denote{\ctx_2} \wedge \len(y_1) = 1
%%%% TMI \]
%%%% TMI %
%%%% TMI and
%%%% TMI \[
%%%% TMI \denote{\heap_3} = \denote{\heap_1}
%%%% TMI                      \hpjoin
%%%% TMI                      \seplista{A}{\addr{\y}}{y_1}.
%%%% TMI \]
%%%% TMI 
%%%% TMI The folding lemma allows us to interpret the heap folding judgement as
%%%% TMI existential generalization in separation logic proofs.
%%%% TMI %
%%%% TMI Intuitively, the judgement walks the non-$\vnull$ references starting
%%%% TMI from a given location, building a pure \emph{snapshot} that will be
%%%% TMI the existential witness that satisfies the given invariant.
%%%% TMI 
%%%% TMI The statement and procedure typing theorems say that we can translate a typing derivation
%%%% TMI into a separation logic proof.
%%%% TMI %
%%%% TMI The proofs are built by induction on the type judgement derivation.
%%%% TMI %
%%%% TMI By the subtyping lemmas, subtype checks become applications of the rule of consequence.
%%%% TMI %
%%%% TMI Heap folding checks become existential generalization.
%%%% TMI 
%%%% TMI 
%%%% TMI \subsection{Subtyping}
%%%% TMI %
%%%% TMI At \cref{line:ex4return}, the type system checks that the returned value, \y,
%%%% TMI is a subtype of \code{insert}'s declared return value.
%%%% TMI %
%%%% TMI Morever, the type system checks that the heap at
%%%% TMI \cref{line:ex4return}, $\heap_3$, is a subtype of the output heap
%%%% TMI specified by \code{insert}.
%%%% TMI %
%%%% TMI These subtyping judgements check the validity of the formulas
%%%% TMI %
%%%% TMI \begin{align*}
%%%% TMI \denote{\ctx_3} &\Rightarrow (\y = \addr{\y}) \Rightarrow (\y = \addr{\y}) \\
%%%% TMI \denote{\ctx_3} & \Rightarrow \denote{\heap_3} \Rightarrow (
%%%% TMI \denote{\hplocty{\addr{y}}{y_1}{\reftp{\tlist{A}}{\len(\vv) = 1 + \len(x)}}}
%%%% TMI \end{align*}
%%%% TMI %
%%%% TMI which hold due to the previous derivations and the fact that
%%%% TMI $\len(\vnull) \doteq 0$.
%%%% TMI 
%%%% TMI We have thus illustrated several key features of our type context
%%%% TMI interpretation.
%%%% TMI %
%%%% TMI First, subtyping judgements in \toolname correspond to application of the rule of
%%%% TMI consequence from Hoare logic.
%%%% TMI %
%%%% TMI Second, the heap folding relation in \toolname corresponds to existential
%%%% TMI generalization.
%%%% TMI %
%%%% TMI Thus, type derivations in \toolname have a corresponding proof in
%%%% TMI separation logic.
%%%% TMI 
%%%% TMI \showsubtyping
%%%% TMI 
%%%% TMI In particular, the translation to separation logic means that if 
%%%% TMI $\issubtype{\ctx}{}{\heap_1}{\heap_2}$, then for each $\loc \in \dom{\heap_2}$,
%%%% TMI $\denote{\ctx} \Rightarrow \sprop{\ty_1}{x} \Rightarrow \sprop{\ty_2}{x}$,
%%%% TMI where $\hplocty{\loc}{x}{\ty_i} \in \heap_i$.
%%%% TMI %
%%%% TMI This lemma corresponds to the use of the rule of consequence in separation logic proofs.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End: 


==> syntaxlang.tex <==
\begin{figure}[t!]
\begin{minipage}{0.45\textwidth}
  \begin{tabular}{l >{$}l<{$} >{$}l<{$}}
\emph{\textbf{Expressions}} & \expr ::= &
                   \vnum 
           \spmid  \vtrue \spmid \vfalse\\
& &          \spmid \vnull
           \spmid  \vref_\loc
           \spmid  \evar\\
& &         \spmid  \expr \op \expr \\[0.01in]
\emph{\textbf{Statements}} & \stmt ::= &
                       \stmt; \stmt 
            \spmid      \evar = \expr\\
& &            \spmid      y = \access{\evar}{\field}
            \spmid      \access{\evar}{\field} \ifappendix =_z \else = \fi \expr\\
& &         \spmid      \ite{\expr}{\stmt}{\stmt}
            \\
           &&
            \spmid      \return{\expr}
           \spmid     \evar \ifappendix =_z \allocl{\loc}{\many{\field:\expr}} 
                              \else = \alloc{\many{\field:\expr}} \fi 
            \spmid      \evar = \funcall{\many{\expr}}
            \\
           &&
            \spmid      \ifappendix \unwindBind{\loc}{\many{x}} \else \unwind{\loc} \fi
            \spmid      \ifappendix \windBind{\loc}{x} \else \wind{\loc} \fi
            \spmid      \ifappendix \concBind{\expr}{z} \else \conc{\expr} \fi
          %%%%%%%%%%%
          \ifappendix
           \spmid     \pad{\loc}{x}
          \fi\\[0.02in]
\emph{\textbf{Programs}} & \prog ::= & \many{\fundecl{f}{\many{\evar}}}
\end{tabular}
\begin{center}
$\vnum \in \text{Integer Constants},\ x,y,f \in \text{Identifiers}, \ \vref_\loc \in \text{Reference Constants},\ \op \in \{+, -, \ldots\}$
\end{center}
  \ifappendix
  \captionof{figure}{Syntax of annotated \lang programs}
  \label{fig:annotsyntax}
  \else
  \captionof{figure}{Syntax of \lang programs}
  \label{fig:syntax}
  \fi
\end{minipage}
\begin{minipage}{0.45\textwidth}
\begin{tabular}{l>{\ } >{$}l<{$} >{$}l<{$} >{$}l<{$}}
\textbf{Primitive Types} & \tprim ::= & 
                    \tint
            \spmid  \tbool
            \spmid  \tvar
            \spmid  \tnull
            \spmid  \tref{\loc}
            \spmid  \trefm{\loc}
            \\[0.01in]
\textbf{Types} & \tbase ::= &
                  \tprim
           \spmid \tyapp{\tycon}{\many{\ty}}
           \spmid \tgenobj{\field}{\ty}\\[0.01in]
\textbf{Refined Types} & \ty ::= & \reft\\[0.01in]
\textbf{Type Definition} & \tycon ::=    & 
                      \tydef{\tyapp{\tycon}{\many{\tvar}}}
                            {\heap}
                            {\evar}
                            {\tobj{\many{f:\ty}}}\\[0.01in]
\textbf{Heaps} & \heap ::= & \hpemp 
           \spmid \heap\hpjoin\hplocty{\loc}{\evar}{\tyapp{\tycon}{\many{\ty}}}
           \spmid \heap\hpjoin\hplocty{\loc}{\evar}{\tgenobj{\field}{\ty}}
    \\[0.01in]
\textbf{Function Types} & \funschema ::= & 
\quant{\many{\loc,\tvar}} \funty{\many{\tybind{\evar}{\ty}}}{\heap}{\equant{\many{\loc'}}\tybind{\evar'}{\ty'}}{\heap'}\\[0.01in]
\textbf{Measure Expressions} & \mexp ::= &
c \spmid {x.f} \spmid \mexp \op \mexp \spmid  \fn{f}(\mexp) \spmid \itex{a}{a}{a}\\[0.01in]
\textbf{Measures} & \measure ::= & \measDef{f}{\vnull}{\mexp} \spmid \measDef{f}{x}{\mexp}
\end{tabular}
\captionof{figure}{Syntax of \lang types}
\label{fig:types}
\end{minipage}
\end{figure}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End: 


==> typedefs.tex <==

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "proof_main.tex"
%%% End: 


==> types.tex <==
\begin{figure*}
  \begin{minipage}{\columnwidth}
  \begin{tabular}{l>{$}l<{$} >{$}l<{$} >{$}l<{$}}
    \tprim & ::=    &              & \textbf{Base Types} \\
           &        & \tint        & \emph{Integers} \\
           & \spmid & \tbool       & \emph{Booleans} \\
           & \spmid & \tvar        & \emph{Type Variables} \\
           & \spmid & \tnull& \emph{Null} \\
           & \spmid & \tref{\loc} & \emph{References} \\
           & \spmid & \tun{\reftp{\tref{\loc}}{p}}{\reftp{\tnull}{q}}\\
    \\[0.05in]
  
    \tbase & ::= & & \textbf{Unrefined Type}\\
           & \spmid & b &\emph{Base Type}\\
           & \spmid & \tyapp{\tycon}{\many{\ty}} & \emph{Type Constructors} \\
           & \spmid & \tgenobj{\field}{\ty} & \emph{Records}\\

    % \\[0.05in]
  \end{tabular}
  \end{minipage}
  \begin{minipage}{\columnwidth}
  \begin{tabular}{l>{$}l<{$} >{$}l<{$} >{$}l<{$}}
    \tycon & ::= & \tydef{\tyapp{\tycon}{\many{\tvar}}}
                         {\heap}
                         {\evar}
                         {\tobj{\many{f:\ty}}} & \textbf{Type Definition} \\
    \\[0.05in]

    \ty & ::=  &  \reft      &  \textbf{Refinement Types} \\

    \\[0.05in]
    \heap  & ::=   & & \textbf{Heaps}\\
           &       & \hpemp & \emph{Empty Heap} \\
           & \spmid& 
  \heap\hpjoin\hplocty{\loc}{\evar}{\tyapp{\tycon}{\many{\ty}}} & \emph{Type Application}            \\
           & \spmid& 
  \heap\hpjoin\hplocty{\loc}{\evar}{\tgenobj{\field}{\ty}} & \emph{Record}            \\

    \\[0.05in]
    \funschema & ::= &
\quant{\many{\loc,\tvar}}% \quant{\many{\tvar}}
\funty{\many{\tybind{\evar}{\ty}}}{\heap}{\tybind{\evar'}{\ty'}}{\heap'}
      % \quant{\many{\tvar}}\quant{\many{\loc}}
      %    \funty{\many{\evar:\ty}}{\heap}{\ty}{\heap} 
& \textbf{Function Schemas}  \\
  \end{tabular}
  \end{minipage}
  \caption{\lang types}
  \label{fig:types}
\end{figure*}

%%% Local Variables: 
%%% mode: latex
%%% eval: (TeX-PDF-mode 1)
%%% TeX-master: "main.tex"
%%% End: 

